COPlanner: Plan to Roll Out Conservatively but to Explore Optimistically for Model-Based RL

Dyna-style model-based reinforcement learning contains two phases: model rollouts to generate sample for policy learning and real environment exploration using current policy for dynamics model learning. However, due to the complex real-world environment, it is inevitable to learn an imperfect dynamics model with model prediction error, which can further mislead policy learning and result in sub-optimal solutions. In this paper, we propose $\texttt{COPlanner}$, a planning-driven framework for model-based methods to address the inaccurately learned dynamics model problem with conservative model rollouts and optimistic environment exploration. $\texttt{COPlanner}$ leverages an uncertainty-aware policy-guided model predictive control (UP-MPC) component to plan for multi-step uncertainty estimation. This estimated uncertainty then serves as a penalty during model rollouts and as a bonus during real environment exploration respectively, to choose actions. Consequently, $\texttt{COPlanner}$ can avoid model uncertain regions through conservative model rollouts, thereby alleviating the influence of model error. Simultaneously, it explores high-reward model uncertain regions to reduce model error actively through optimistic real environment exploration. $\texttt{COPlanner}$ is a plug-and-play framework that can be applied to any dyna-style model-based methods. Experimental results on a series of proprioceptive and visual continuous control tasks demonstrate that both sample efficiency and asymptotic performance of strong model-based methods are significantly improved combined with $\texttt{COPlanner}$.

==> corl_2023_ws/1_intro.tex <==
\section{Introduction}\label{sec:intro}

\begin{wrapfigure}[10]{R}{5cm}
\vspace{-17pt}
\includegraphics[width=5cm]{MBRL-model based planning/exp/exp_total.png}
\vspace{-20pt}
\caption{Mean performance of \ouralgo compared with baselines across 3 diverse benchmarks.
% The performance shows a significant improvement. 
% In visual DMC tasks, COPlanner represents COPlanner-DreamerV3. In other two domains, COPlanner means COPlanner-MBPO.
}\label{fig: exp_total}
% \vspace{-15pt}
\end{wrapfigure}
Model-Based Reinforcement Learning (MBRL) has emerged as a promising approach to improve the sample efficiency of model-free RL methods. 
Most MBRL methods contain two phases that are alternated during training: 1) the first phase where the agent interacts with the real environment using a policy to obtain samples for dynamics model learning; 2) the second phase where the learned dynamics model rolls out to generate massive samples for updating the policy.
Consequently, learning an accurate dynamics model is critical as the model-generated samples with high bias can mislead the policy learning~\citep{deisenroth2011pilco, wu2022plan}.

\begin{figure}[!htbp]
\centering
\vspace{-15pt}
\includegraphics[width=0.8\textwidth]{MBRL-model based planning/exp/framework_v3.png}
\vspace{-10pt}
\caption{\small{\ouralgo Framework. The most essential part of \ouralgo is the \textit{Uncertainty-aware Policy-Guided MPC (UP-MPC) phase} in which we plan trajectories of length $H$, according to the learned dynamics model and learned policy network $\pi$, to select the action with highest trajectory reward. This UP-MPC phase is implemented differently for the two different purposes: \textit{\textcolor[RGB]{192,0,0}{environment exploration}} v.s. \textit{\textcolor[RGB]{68,114,196}{dynamics model rollouts}}. In \textcolor[RGB]{192,0,0}{environment exploration}, trajectory reward has an uncertainty bonus term to encourage exploring uncertain regions in the environment. In \textcolor[RGB]{68,114,196}{dynamics model rollouts}, trajectory reward, on the contrary, has an uncertainty penalty term to encourage policy learning on confident regions of the learned dynamics model.}}
\vspace{-20pt}
\label{fig:Framwork}
\end{figure}

However, dynamics model errors are inevitable due to the complex real-world environment.
Existing methods try to avoid model errors in two main ways.
1) Design different mechanisms such as filtering out error-prone samples to mitigate the influence of model errors after model rollouts \citep{{buckman2018sample}, {yu2020mopo}, {pan2020trust},{yao2021sample}}. 
2) Actively reduce model errors during real environment interaction through uncertainty-guided exploration \citep{{shyam2019model}, {ratzlaff2020implicit}, {sekar2020planning}, {mendonca2021discovering}}.
While both categories of methods have achieved advancements, each comes with its own set of limitations.
For the first category, although these approaches are shown to be empirically effective, they primarily concentrate on estimating uncertainty at the current step, often neglecting the long-term implications that present samples might have on model rollouts.
Moreover, post-processing samples after model rollouts can compromise rollout efficiency as many model-generated samples are discarded or down-weighted.
As for the second category, it is intrinsically challenging to achieve low model error and high long-term reward without sacrificing the sample efficiency by learning exploration policies.
% The drawback of these methods is that uncertainty-guided exploration may results in excessive investigation of areas with low rewards. 
% Samples derived from these zones will not enhance policy, resulting in low sample efficiency.

% In this paper, we propose \ouralgo, a novel model-based RL framework to improve sample efficiency in MBRL by \textit{conservative} model rollouts and \textit{optimistic} real environment exploration. More specifically, we measure the estimated model uncertainty as a penalty or a bonus on the total planning trajectory rewards for the rollout and real interaction phases respectively. We achieve this by leveraging a policy-guided model-predictive control (MPC) phase on action selection. As shown in Figure~\ref{fig:Framwork}, before each interaction with the dynamics model or the real environment, we first predict the potential future trajectories and corresponding cumulative uncertainties by performing multi-step planning with the current action. Then, Policy-Guided MPC chooses actions that either conservatively roll out imaginary trajectories to avoid model uncertain regions or optimistically explore the real environment. Conservative rollouts and optimistic exploration enjoy, interestingly, a symmetric form which makes our framework easy to implement.

To tackle the aforementioned limitations, we introduce a novel framework, \ouralgo, 
which mitigates the model errors from two aspects: 1) avoid being misled by the existing model errors via conservative model rollouts, and 2) keep reducing the model error via optimistic environment exploration. 
The two aspects are achieved simultaneously by a novel uncertainty-aware multi-step planning method, which requires no extra exploration policy training nor additional samples, resulting in stable policy updates and high sample efficiency.
% which can mitigate the influence of model errors during model rollouts and explore the environment to actively reduce model errors simultaneously by leveraging uncertainty-aware planning.
% which incorporates long-term vision and model uncertainty into action selection. 
% This innovation is unprecedented in the field of model-based RL. 
\ouralgo is structured around three core components: \textit{the Planner}, \textit{conservative model rollouts}, and \textit{optimistic environment exploration}. In the Planner, we employ an \textit{Uncertainty-aware Policy-guided Model Predictive Control} (UP-MPC) to forecast future trajectories in terms of selecting actions and to estimate the long-term uncertainty associated with each action.
% (Sec~\ref{sec: 3.1}).
As shown in Figure~\ref{fig:Framwork}, this long-term uncertainty serves as dual roles.
% tailored to mitigate the effect of model error in the two distinct phases of model-based RL: model rollouts (i.e., policy update) and environment exploration (i.e. model learning). 
% In model rollouts phase, the uncertainty guides the selection of conservative actions (Sec~\ref{sec: 3.2}), while in model learning phase, it steers towards optimistic actions for environment exploration (Sec~\ref{sec: 3.3}).
In the model rollouts phase, the uncertainty acts as a penalty on the total planning trajectory, guiding the selection of conservative actions. 
Conversely, during the model learning phase, it serves as a bonus on the total planning trajectory, steering towards optimistic actions for environment exploration.
% More specifically, we measure the estimated model uncertainty as a penalty or a bonus on the total planning trajectory rewards for the rollout and real interaction phases respectively. 
% As shown in Figure~\ref{fig:Framwork}, before each interaction with the \textcolor[RGB]{68,114,196}{dynamics model} or the \textcolor[RGB]{192,0,0}{real environment}, we first predict the potential future trajectories and corresponding cumulative uncertainties by performing multi-step planning with the current action. 
% Then, the Planner chooses actions that either \textcolor[RGB]{68,114,196}{conservatively roll out imaginary trajectories to avoid model uncertain regions} or \textcolor[RGB]{192,0,0}{optimistically explore the real environment to expand the learned model}.




Compared to previous methods, \ouralgo has the following advantages:
\textbf{(a)} \ouralgo has \textbf{higher exploration efficiency}, as it focuses on investigating high-reward uncertain regions to broaden the dynamics model, thereby preventing unnecessary excessive exploration of areas with low rewards.
\textbf{(b)} \ouralgo has \textbf{higher model-generated sample utilization rate.} Through planning for multi-step model uncertainty estimation, \ouralgo can prevent model rolled out trajectories from falling into uncertain areas, thereby avoiding model errors before model rollouts and improving the utility of model generated samples.
\textbf{(c)} \ouralgo enjoys an \textbf{unified policy framework}. Unlike previous methods \citep{{sekar2020planning}, {mendonca2021discovering}} that require training two separate policies for different usage, \ouralgo only requires training a single policy and we only change the way model-based planning is utilized, thus improving training efficiency and resolving potential policy distribution mismatches. 
\textbf{(d)} \ouralgo ensures \textbf{undistracted policy optimization}. Notably, \ouralgo diverges from existing approaches by not using long-term uncertainty as an intrinsic reward. Instead, the policy's objective remains focused on maximizing environmental rewards, thereby avoiding the introduction of spurious behaviors due to model uncertainty.


\textbf{Summary of Contributions:}
\textbf{(1)} We introduce \ouralgo framework which can mitigate the influence of model errors during model rollouts and explore the environment to actively reduce model errors simultaneously by leveraging our proposed uncertainty-aware policy-guided MPC.
\textbf{(2)} \ouralgo is a plug-and-play framework that can be applicable to any dyna-style MBRL method. 
\textbf{(3)} After being integrated with other MBRL baseline methods, \ouralgo improves the sample efficiency of these baselines by nearly double.
\textbf{(4)} Besides, \ouralgo also significantly improves the performance on a suite of proprioceptive and visual control tasks compared with other MBRL baseline methods (16.9\% on proprioceptive DMC, 59.7\% on MuJoCo, and 23.9\% on visual DMC).
% We propose \ouralgo framework that has a long-term vision for uncertainty estimation.
% This mechanism utilizes the long-term uncertainty for both conservative model rollouts and optimistic environment exploration, thereby addressing the inaccurate learned dynamics model problem in MBRL. 
% \textbf{(2)} More importantly, \ouralgo achieves simultaneously conservative model rollouts and optimistic environment exploration using a single policy, whose learning is not interfered by conservative rollouts or optimistic exploration, in contrast with existing works. 
% \textbf{(3)} \ouralgo is a plug-and-play framework that can be applicable to any dyna-style MBRL method. 
% \textbf{(4)} \ouralgo, combined with the current MBRL methods, significantly improves both the sample efficiency and performance on a suite of proprioceptive and visual control tasks.

==> corl_2023_ws/2_background.tex <==
\section{Preliminaries}
\textbf{Model-based reinforcement learning.}
We consider a Markov Decision Process (MDP) defined by the tuple $(\mathcal{S}, \mathcal{A}, \mathcal{T},\rho_0, r, \gamma)$, 
where $\mathcal{S}$ and $\mathcal{A}$ are the state space and action space respectively, $\mathcal{T}(s^{\prime}|s,a)$ is the transition dynamics, $\rho_0$ is the initial state distribution, $r(s,a)$ is the reward function and $\gamma$ is the discount factor.
In model-based RL, the transition dynamics $T$ in the real world is unknown, and we aim to construct a model $\hat{T}(s^{\prime}|s,a)$ of transition dynamics and use it to find an optimal policy $\pi$ which can maximize the expected sum of discounted rewards,
\begin{equation}
\label{eq_MBRLgoal}
\pi = \mathop{\arg\!\max}_{\pi}\mathbb{E}_{{s_{t}\sim \hat{T}(\cdot|s_{t-1},a_{t-1})} \atop{a_t \sim \pi(a|s_t)}}\left[\sum_{t=0}^{\infty}\gamma^t r(s_t, a_t)\right].
\end{equation}

\textbf{Model predictive control.}
Model predictive control (MPC) has a long history in robotics and control systems \citep{{garcia1989model}, {qin2003survey}}.
MPC find the optimal action through trajectory optimization. 
Specifically, given the transition dynamics $T$ in the real world, the agent obtains a local solution at each step $t$ by estimating optimal actions over a finite horizon $H$ (i.e., from $t$ to $t+H$) and executing the first action $a_t$ from the computed optimal sequence at time step $t$:
\begin{equation}
\label{eq_MPCgoal}
a_t = \mathop{\arg\!\max}_{a_{t:t+H}}\mathbb{E}\left[\sum_{i=t}^H \gamma^i r(s_i, a_i)\right], s_i \sim T(\cdot|s_{i-1}, a_{i-1}),
\end{equation}
where $\gamma$ is typically set to 1.
In model-based control methods, the transition dynamics $T$ is %always
simulated by the learned dynamics model $\hat{T}$ \citep{{chua2018deep}, {wang2019exploring}, {hansen2022temporal}}.

==> corl_2023_ws/3_method.tex <==
\section{The \ouralgo Framework}
% In this section, we will introduce our \ouralgo framework. 
% We first present the core part of \ouralgo called Policy-Guided model predictive control, or Policy-Guided MPC.
% Then we introduce the specific forms of Policy-Guided MPC for different purposes at different stages, namely model rolling out conservatively and exploring the environment optimistically.
% As motivated in previous sections that being able to avoid or reduce model error dueing planning and model learning is the major issue we aim to tackle. 
% Our idea is to adjust actions according to model uncertainty based on the curre t learned transition dynamics and current policy. the major novelty includes (1) how to calculate model uncertainty, (2) how to adjust the action selection during the two differencet stages of the model-based RL, and (3) how to select action that has a long-term vision. In this section, we will introduce a planner, which concerns the 3rd novelty. how to use this planner, which concerns the second novelty, will be introduced in the following subsections.

In this section, we will introduce \ouralgo framework. 
\ouralgo consists of three components: the Planner, conservative model rollouts, and optimistic environment exploration. 
Within the Planner, we propose using an Uncertainty-aware Policy-guided MPC to predict potential future trajectories when selecting different actions under the current state and estimate the long-term uncertainty associated with each action, which will be introduced in Sec~\ref{sec: 3.1}.
Depending on the phase, this long-term uncertainty is used to further guide the selection of conservative actions for policy learning or optimistic actions for environment exploration which will be introduced in Sec~\ref{sec: 3.2} and Sec~\ref{sec: 3.3}. 
% It's worth noting that, unlike previous works, in our framework, the long-term uncertainty is not used as an intrinsic reward for policy training.
% The policy's objective remains to maximize the environment reward, which mitigates any potential issues with the policy learning spurious behaviors due to model uncertainty.
% The pseudocode of \ouralgo is shown in Algorithm~\ref{coplanner wrapper}, and a more detailed figure is shown in Appendix~\ref{app: framework_figure}.




\subsection{``The Planner'': Uncertainty-Aware Policy-Guided MPC}\label{sec: 3.1}

\begin{wrapfigure}{r}{0.45\textwidth}
\vspace{-13pt}
\includegraphics[width=0.45\textwidth]{MBRL-model based planning/exp/MPC_v2.png}
\vspace{-15pt}
\caption{The Planner.\label{fig:mpc}}
\vspace{-15pt}
\end{wrapfigure}
In this section, we present the core part of our proposed framework which is called Uncertainty-aware Policy-guided MPC (UP-MPC). 
% \fhc{As motivated in previous sections that being able to avoid or reduce model error dueing planning and model learning is the major issue we aim to tackle. Our idea is to adjust actions according to model uncertainty based on the curret learned transition dynamics and current policy. the major novelty includes (1) how to calculate model uncertainty, (2) how to adjust the action selection during the two differencet stages of the model-based RL, and (3) how to select action that has a long-term vision. In this section, we will introduce a planner, which concerns the 3rd novelty. how to use this planner, which concerns the second novelty, will be introduced in the following subsections. }
Inspired by MPC, we apply the random shooting method \citep{rao2009survey} to introduce a long-term vision. % in MPC.
Specifically, given the current state $s_t$, before each interaction with the model or real environment, we first generate an action candidate set containing $K$ actions using the policy: $\bm{a_t} = \{a_t^{(1)}, a_t^{(2)}, ..., a_t^{(k)}\}$.
Then, for each action candidate, we perform $H_p$-step planning and calculate the reward $r$, and model uncertainty $u$ for each step.
Finally, we select the action according to accumulated reward and model uncertainty, (to interact with the learned dynamics for the model rollouts or to interact with the environment for the model learning),  
% This selected action will be used for different purposes: to interact with the model for the model rollouts phase or to interact with the environment for the environment exploration. 
as will be discussed in details in Sec~\ref{sec: 3.2} and Sec~\ref{sec: 3.3}.

Incorporating model uncertainty is crucial for action selection to compensate for model error.
As illustrated in Algorithm~\ref{alg: MPC}, we calculate the model uncertainty $u$ through the model disagreement \citep{pathak2019self} method. 
Model disagreement is closely related to model learning and is currently the most common way to estimate model uncertainty in MBRL \citep{{yu2020mopo}, {kidambi2020morel}, {pan2020trust}, {sekar2020planning}, {yao2021sample}, {mendonca2021discovering}}. 
We train a dynamics model ensemble $\hat{T}_{\theta} = \{ \hat{T}^{(1)}_{\theta}, \hat{T}^{(2)}_{\theta}, ..., \hat{T}^{(n)}_{\theta} \}$ to predict the next state given the current state-action pair $(s_t, a_t)$ as input.
Utilizing the ensemble, we approximate the model uncertainty by calculating the variance over predicted states of the different ensemble members.
This estimation closely represents the expected information gain \citep{pathak2019self}:
\vspace{-3pt}
\begin{equation}
\label{eq_model_disagreement}
u(s_t, a_t) = \frac{1}{N-1}\sum_n (\hat{T}^{(n)}_{\theta}(s_t, a_t) - \mu^{\prime})^2, \quad \mu^{\prime} = \frac{1}{N}\sum_n \hat{T}^{(n)}_{\theta}(s_t, a_t).
\end{equation}
\vspace{-10pt}

See Figure~\ref{fig:mpc} for the illustration of the process.
The pseudocode for the Planner, i.e., the UP-MPC process, is summarized in Algorithm~\ref{alg: MPC}.

\vspace{-10pt}
\begin{algorithm}[!htbp]
\caption{The Planner: \textbf{UP-MPC}\;\big($\pi_\phi$, $s$, $\hat{T}_{{\theta}}$, $K$, $H$, $\alpha$\big)}
\begin{algorithmic}[1]
\REQUIRE Policy $\pi_\phi$, State $s$, learned dynamics model $\hat{T}_{{\theta}}$, number of candidates actions $K$, planning horizon $H_p$, optimistic/conservative parameter $\alpha$ \
\STATE Initialize $R^{(k)}=0$ for $k=1,..., K$, $s^{(k)}_0=s$ for $k=1,..., K$
\FOR {$k=1$ to $K$}
\FOR{$t=0$ to $H_p-1$}
    \STATE Sample $a^{(k)}_t\sim \pi_\phi(\cdot|s^{(k)}_t)$
    \STATE Rollout dynamics model $r^{(k)}_{t} = \hat{R}(\cdot|s^{(k)}_t, a^{(k)}_t), \; s^{(k)}_{t+1}\sim \hat{T}_{{\theta}}(\cdot|s^{(k)}_t, a^{(k)}_t)$
    \STATE Compute model uncertainty $u^{(k)}_t$ according to Eq.~\ref{eq_model_disagreement}
    \STATE $R^{(k)} = R^{(k)} + r^{(k)}_t + \alpha u^{(k)}_t$
    \ENDFOR
\ENDFOR
\STATE  Select $k^*=\argmax_{k=1,..., K}R^{(k)}$
\RETURN $a^{({k^*})}_0$
\end{algorithmic}
\label{alg: MPC}
\end{algorithm}
\vspace{-5pt}

Although in  Algorithm~\ref{alg: MPC} 
% for simplicity of illustration, 
model uncertainty $u$ is implemented through model disagreement, our proposed 
UP-MPC is a generic framework, any method for calculating intrinsic rewards to encourage exploration can be embedded into our framework for computing $u$. 
In Appendix~\ref{app: exp_uncert} we provide an ablation study of uncertainty estimation methods to further illustrate this point.
% Here we only introduce the model disagreement \citep{pathak2019self} method we used. 


\subsection{Conservative model rollouts}\label{sec: 3.2}

In model-based RL, due to the limited samples available for model learning, model prediction errors are inevitable. 
If a policy is trained using model-generated samples with a large error, these samples will not provide correct gradient and may mislead the policy update. 
Previous methods estimate the model uncertainty of each sample after generation and re-weight or discarded samples with high uncertainty. 
However, re-weighting samples based on uncertainty still leads to samples with high uncertainty participating in the policy learning process, while filtering requires manually setting an uncertainty threshold, and determining the optimal threshold is difficult. 
Discarding too many samples can result in inefficient rollouts.

% Since processing samples after generation is inefficient, can we predict the impact of an action on future rollouts before executing it, thereby avoiding generating high uncertainty samples? The answer is yes. 
We apply our Planner to plan for maximizing the future reward while minimizing the model uncertainty during model rollouts before executing the action. 
After calculating the reward and model uncertainty for the $H_p$-step trajectories of $K$ action candidates (line 5 and 6 in Algorithm~\ref{alg: MPC}),  
we replace $\alpha=\textcolor{blue}{-\alpha_c}$, for a positive $\alpha_c>0$ at line 7 in Algorithm~\ref{alg: MPC}.
Mathematically, %this choice of $\alpha=-\alpha_c$ means that 
we select the action according to Eq.~\ref{eq_act_rollout} to interact with the model for model rollouts:
\begin{equation}\label{eq_act_rollout}
\resizebox{\hsize}{!}{$
a = \mathop{\arg\!\max}_{a_t \in \bm{a_t}} \left[ r(s_t, a_t) + \sum_{i=1}^{H_p} r(\hat{s}_{t+i}, \pi(\hat{s}_{t+i})) \textcolor{blue}{- \alpha_c} \sum_{i=1}^{H_p} u(\hat{s}_{t+i}, \pi(\hat{s}_{t+i})) \right], \hat{s}_{t+i} \sim \hat{T}(\cdot|\hat{s}_{t+i-1}, a_{t+i-1}).
$}
\end{equation}
The negative $-\alpha_c$ is a coefficient that adds the model uncertainty as a penalty term to the trajectory total reward. 
By employing this approach, we can prevent model rollout trajectories from falling into model-uncertain regions while obtaining samples with higher rewards.


\subsection{Optimistic environment exploration}\label{sec: 3.3}

In addition to model rollouts, another crucial part of MBRL is interacting with the real environment to obtain samples to improve the dynamics model. 
Since the main purpose of MBRL is to improve sample efficiency, we should acquire more meaningful samples for improving the dynamics model within a limited number of interactions. 
Therefore, unlike previous methods that merely aimed to thoroughly explore the environment to obtain a comprehensive model \citep{{shyam2019model}, {ratzlaff2020implicit}, {sekar2020planning}}, we do not expect the dynamics model to learn all samples in the state space. This is because many low-reward samples do not contribute to policy improvement. 
Instead, we hope to obtain samples with both high rewards and high model uncertainty to sufficiently expand the model and reduce model uncertainty.

Similar to model rollouts, we also employ our Planner in the process of selecting actions when interacting with the environment. 
However, the difference lies in that we  replace $\alpha=\textcolor{red}{\alpha_o}$, for a positive $\alpha_o>0$ at line 7 in Algorithm~\ref{alg: MPC}.
Mathematically, we choose the action with both high cumulative rewards and model uncertainty according to Eq.~\ref{eq_act_planning}, which is a symmetric form of Eq.~\ref{eq_act_rollout}. $\alpha_o$ is a hyperparameter to balance the reward and exploration.
Such an action can guide the trajectory towards regions with high rewards and model uncertainty in the real environment, thereby effectively expanding the learned dynamics model. 
\begin{equation}
\label{eq_act_planning}
\resizebox{\hsize}{!}{$
a = \mathop{\arg\!\max}_{a_t \in \bm{a_t}} \left[ r(s_t, a_t) + \sum_{i=1}^{H_p} r(\hat{s}_{t+i}, \pi(\hat{s}_{t+i})) \textcolor{red}{+ \alpha_o} \sum_{i=1}^{H_p} u(\hat{s}_{t+i}, \pi(\hat{s}_{t+i})) \right], \hat{s}_{t+i} \sim \hat{T}(\cdot|\hat{s}_{t+i-1}, a_{t+i-1})
$}
\end{equation}

In summary, by simultaneously using conservative model rollouts and optimistic environment exploration, \ouralgo effectively alleviates the model error problem in MBRL. 
As we will show in \cref{sec: exp}, this is of great help in improving the sample efficiency and performance.
The pseudocode of \ouralgo is shown in Algorithm~\ref{coplanner wrapper}, and a more detailed figure is shown in Appendix~\ref{app: framework_figure}.
Very importantly, \ouralgo achieves both conservative model rollouts and optimistic environment exploration using a single policy. Different from prior exploration methods, the policy that \ouralgo learns does not have to be an ``exploration'' policy which is inevitably suboptimal.


\begin{algorithm}[htbp]
\caption{Main Algorithm: \ouralgo}
\begin{algorithmic}[1]
\REQUIRE Interaction epochs $I$, rollout horizon $H_r$, planning horizon $H_p$, number of candidates actions $K$, conservative rate $\alpha_c$, optimistic rate $\alpha_o$ \
\STATE Initialize policy $\pi_\phi$, dynamics model $\hat{T}$, real sample buffer $\mathcal{D}_{\textit{e}}$, model sample buffer $\mathcal{D}_{\textit{m}}$
\FOR{$I$ epochs}
    % \FOR{$t=1$ to $T$}
    \WHILE{not Done}
    \STATE Select action $a_t = \textbf{UP-MPC}\big(\pi_\phi, s_t, \hat{T}_{{\theta}}, K, H_p, \textcolor{red}{\alpha_o}\big)$
    \STATE Execute in real environment, add $(s_t, a_t, r_t, s_{t+1})$ to $\mathcal{D}_{\textit{e}}$ \
    \STATE Train dynamics model $\hat{T}_{{\theta}}$ with $\mathcal{D}_{\textit{e}}$ \
    \FOR{$M$ model rollouts}
    \STATE Sample initial states from real sample buffer $\mathcal{D}_{\textit{e}}$ \
        \FOR{$h=0$ to $H_r$}
            \STATE Select action $\displaystyle \hat{a}_{t+h} = \textbf{UP-MPC}\big(\pi_\phi, \hat{s}_h, \hat{T}_{{\theta}}, K, H_p, {\textcolor{blue}{-\alpha_c}}\big)$
            \STATE Rollout learned dynamics model and add to $\mathcal{D}_{\textit{m}}$
        \ENDFOR
    \ENDFOR
    \STATE Update current policy $\pi_{{\phi}}$ with $\mathcal{D}_m$ \
    \ENDWHILE
\ENDFOR
% \ENDFOR
\end{algorithmic}
\label{coplanner wrapper}
\end{algorithm}
\vspace{-5pt}

==> corl_2023_ws/5_experiment.tex <==
\section{Experiment}
\label{sec: exp}

In this section, we combine \ouralgo with strong MBRL baseline methods and conduct experiments on both proprioceptive control environments and visual control environments to demonstrate the effectiveness of our method. 
Due to space constraints, further discussions about the method and ablation studies can be found in Appendix~\ref{App: exp}.

\subsection{Experiment on proprioceptive control tasks}
\label{subsec: prop exp}
\textbf{Baselines}: 
In this section, we conduct experiments to demonstrate the effectiveness of \ouralgo on proprioceptive control MBRL methods. 
We combine \ouralgo with MBPO~\citep{janner2019trust}, the most classic method in proprioceptive control dyna-style MBRL, and we name the combined method as \textbf{COPlanner-MBPO}. 
The implementation details can be found in Appendix~\ref{app: implementation details}.
Consequently, \textbf{MBPO} naturally becomes one of our baselines. 
The other two baselines are \textbf{P2P-MPC}~\citep{wu2022plan} and \textbf{MEEE}~\citep{yao2021sample}.
These two methods also aim to mitigate the impact of model errors in model-based RL.
More details of P2P-MPC and MEEE can be found in Section~\ref{sec: related work}.
We also provide comparison with more proprioceptive control MBRL methods in Appendix~\ref{app: exp_pmbrl}.

\textbf{Environment and hyperparameter settings}:
We conduct experiments on 8 proprioceptive continuous control tasks of DeepMind Control (DMC) and 4 proprioceptive control tasks of MuJoCo.
MBPO trains an ensemble of 7 networks as the dynamics model while using the Soft Actor-Critic (SAC) as the policy network. 
In COPlanner-MBPO, we adopt the setting of MBPO and directly use the dynamics model ensemble to calculate model uncertainty for action selection in Policy-Guided MPC.
For hyperparameter setting, we set optimistic rate $\alpha_o$ to be 1, conservative rate $\alpha_c$ to be 2 in most tasks. 
We set action candidate number $K$ and planning horizon $H_p$ equal to 5 in all tasks.
The specific setting are shown in the Appendix~\ref{app: hyper_vdmc}. 

\begin{figure}[!htbp]
\centering
\includegraphics[width=0.9\textwidth]{MBRL-model based planning/exp/exp_pinput.png}
\vspace{-5pt}
\caption{Experiment results of COPlanner-MBPO and other three baselines on proprioceptive control environments. The curves in the first eight figures originate from DM Control tasks, while those in the last four are from MuJoCo tasks. The results are averaged over 8 random seeds, and shaded regions correspond to the $95\%$ confidence interval among seeds.
During evaluation, for each seed of each method, we test for up to 1000 steps in the test environment and perform 10 evaluations to obtain an average value. 
The evaluation interval is every 1000 environment steps.
}
\vspace{-10pt}
\label{fig: pinput_comparison}
\end{figure}

% \begin{figure}[!htbp]
% \centering
% \includegraphics[width=\textwidth]{MBRL-model based planning/exp/exp_mujoco.png}
% \vspace{-15pt}
% \caption{Experiment results of COPlanner-MBPO and other three baselines on MuJoCo. The results are averaged over 4 random seeds, and shaded regions correspond to the $95\%$ confidence interval among seeds.}
% \vspace{-20pt}
% \label{fig: mujoco_comparison}
% \end{figure}

\textbf{\ouralgo significantly improves the sample efficiency and performance of MBPO}:
Through the results in Figure~\ref{fig: pinput_comparison} we can find that both sample efficiency and performance of MBPO have a significant improvement after combining \ouralgo.
\textbf{(a) Sample efficiency}:
In proprioceptive control DMC, the sample efficiency is improved by $40\%$ on average compared to MBPO. 
For example, in the Walker-walk task, MBPO requires 100k steps for the performance to reach 700, while COPlanner-MBPO only needs approximately 60k steps.
In more complex MuJoCo tasks, the improvement brought by \ouralgo is even more significant.
Compared to MBPO, the sample efficiency of COPlanner-MBPO has almost doubled.
\textbf{(b) Performance}:
From the performance perspective, as shown in Figure~\ref{fig: exp_total}, the performance of MBPO has improved by $16.9\%$ after combining \ouralgo. 
Moreover, it is worth noting that our method successfully solves the Walker-run task, which MBPO fails to address, further demonstrating the effectiveness of our proposed framework.
In MuJoCo tasks, the average performance at 150k environment steps has increased by $59.7\%$.
Besides, COPlanner-MBPO also outperforms other two baselines.

\subsection{Experiment on visual control tasks}

\textbf{Baselines}: 
We conduct experiments to demonstrate the effectiveness of our proposed framework on visual control environments.
We integrate our algorithm with DreamerV3 \citep{hafner2023mastering}, the state-of-the-art Dyna-style model-based RL approach recently introduced for visual control.
% We combine \ouralgo with DreamerV3 \citep{hafner2023mastering}, the SOTA dyna-style model-based RL for visual control proposed recently.
The implementation details can be found in Appendix~\ref{app: implementation details}.
We choose LEXA  \citep{mendonca2021discovering} as our another baseline.
LEXA uses Plan2Explore \citep{sekar2020planning} as intrinsic reward to explore the environment and learn a world model, then using this model to train a policy to solve diverse tasks such as goal achieving.
Here we adopt LEXA on DreamerV3 to address continuous control tasks and name it as LEXA-DreamerV3.
Since pure exploration base on Plan2Explore is sample inefficient for model learning when solving specific tasks, we use the real reward provided by environment as extrinsic reward and add it to intrinsic reward provided by Plan2Explore to train the explorer.
We call this baseline LEXA-reward-DreamerV3.
We also provide comparison with more visual control MBRL methods including TDMPC~\citep{hansen2022temporal} and PlaNet~\citep{hafner2019learning} in Appendix~\ref{app: exp_vmbrl}.

\begin{figure}[!htbp]
\centering
\includegraphics[width=0.9\textwidth]{MBRL-model based planning/exp/exp_dreamerv3.png}
\vspace{-5pt}
\caption{Experiment results of COPlanner-Dreamerv3 and other three baselines on pixel-input DMC. The results are averaged over 8 random seeds, and shaded regions correspond to the $95\%$ confidence interval among seeds.
During evaluation, for each seed of each method, we test for up to 1000 steps in the test environment and perform 10 evaluations to obtain an average value. 
The evaluation interval is every 1000 environment steps.
}
\vspace{-10pt}
\label{fig: visualinput_comparison}
\end{figure}


\textbf{Environment and hyperparameter settings}:
We use 8 visual control tasks of DMC as our environment.
In COPlanner-DreamerV3, we learn a latent one-step prediction dynamics model as Plan2Explore~\citep{sekar2020planning}, the ensemble size is 8.
We set action candidate number $K$ and planning horizon $H_p$ equal to 4 in all tasks.
For optimistic rate $\alpha_o$ and conservative rate $\alpha_c$, we set them to be 1 and 0.5, respectively.
All other hyperparameters remain consistent with the original DreamerV3 paper.
% due to the complexity of the visual control environment, we tune $\alpha_o$ and $\alpha_c$ for each task separately. 
% The specific setting can be found in the Appendix~\ref{app: hyper_pdmc}. 

\textbf{\ouralgo significantly improves the sample efficiency and performance of DreamerV3}:
From the experiment results in Figure~\ref{fig: visualinput_comparison}, we observe that COPlanner-DreamerV3 improves the sample efficiency and performance significantly over DreamerV3.
The sample efficiency of COPlanner-DreamerV3 is more than twice that of DreamerV3, and the performance is improved by 23.9\%.
Besides, LEXA-DreamerV3 has a low sample efficiency and do not perform well.
This demonstrates the limitation of pure exploration when the goal is to solve specific tasks instead of learning a dynamics model applicable to a variety of tasks.
After adding real reward as extrinsic reward for explorer learning, LEXA-reward-DreamerV3 delivers performance comparable to DreamerV3 in most environments.
It outperforms DreamerV3 in Cartpole-swingup-sparse and Hopper-stand.
However, its performance and sample efficiency are still worse than COPlanner-DreamerV3, further indicates the effectiveness of \ouralgo.

==> corl_2023_ws/6_relatedworks.tex <==
\section{Related work}\label{sec: related work}


\textbf{Mitigating model error by improving rollout strategies.} Prior methods primarily focus on using dynamics model ensembles \citep{{kurutachmodel}, {chua2018deep}} to assess model uncertainty of samples after they were generated by the model, and then 
apply weighting techniques \citep{{buckman2018sample}, {yao2021sample}}, penalties \citep{{kidambi2020morel}, {yu2020mopo}}  or filtering \citep{{pan2020trust}, {wang2022sample}} to those high uncertainty samples to mitigate the influence of model error. 
These methods only quantify uncertainty after generating the samples 
and since their uncertainty metrics are based on the current step and are myopic, these metrics can not evaluate the potential influence of the current sample on future trajectories. 
Therefore, they fail to prevent the trajectories, which is generated through model rollout on the current policy, from entering high uncertainty regions, eventually leading to a failed policy update. 
Wu et al.~\citep{wu2022plan} proposed Plan to Predict (P2P), which reverses the roles of the model and policy during model learning to learn an uncertainty-foreseeing model, aiming to avoid model uncertain regions during model rollouts. Combined with MPC, their method achieved promising results. 
However, their approach lacks effective exploration of the environment.
Branched rollout \citep{janner2019trust} and bidirectional rollout \citep{lai2020bidirectional} take advantage of small model errors in the early stages of rollouts and uses shorter rollout horizons to avoid model errors, but these approaches limit the planning capabilities of the learned dynamics model.
Besides, different model learning objectives \citep{{shen2020model}, {eysenbach2022mismatched}, {wang2022live}, {zheng2023model}} are designed to solve objective mismatch \citep{lambert2020objective} in model-based RL and further mitigate model error during model rollouts.


\textbf{Reducing model error by improving environment exploration.} Another approach to mitigate model error is to expand the dynamics model by obtaining more diverse samples through exploration during interactions with the environment. 
However, previous methods mostly focused on pure exploration, i.e., how to make the dynamics model learn more comprehensively \citep{{shyam2019model}, {ratzlaff2020implicit}, {sekar2020planning}, {mendonca2021discovering}, {hu2023planning}}. 
In complex environments, thoroughly exploring the entire environment is very sample-inefficient and not practical in real-world applications. 
Moreover, using pure exploration to expand the model may lead to the discovery of many low-reward samples (e.g., different ways an agent may fall in MuJoCo environment \citep{todorov2012mujoco}), which are not very useful for policy learning. 
Mendonca et al. \citep{mendonca2021discovering} proposed Latent Explorer Achiever (LEXA) which involves a explorer for exploring the environment and one achiever for solving diverse tasks based on collected samples, but the explorer and achiever may experience policy distribution shift under specific single-task settings, causing the achiever to potentially not converge to the optimal solution.


\textbf{Mitigating model error from both sides.} One most relevant work is Model-Ensemble Exploration and Exploitation (MEEE) \citep{yao2021sample} which simultaneously expands the dynamics model and reduces the impact of model error during model rollouts. During the rollout process, it uses uncertainty to weight the loss calculated for each sample to update the policy and the critic. Before interacting with the environment, they first generate $k$ action candidates and then select the action with the highest sum of Q-value and one-step model uncertainty to execute.
However, as we mentioned earlier, weighting samples cannot fundamentally prevent the impact of model errors on policy learning, and it may still mislead policy updates. Moreover, since the one-step prediction error of dynamics models is often small \citep{pan2020trust}, relying only on the sum of Q-values and one-step model uncertainty may not effectively differentiate action candidates. As a result, samples collected during interactions with the environment might not efficiently expand the model.



==> corl_2023_ws/7_conclusion.tex <==
\section{Conclusion and discussion}

We investigate how to effectively address the inaccurate learned dynamics model problem in MBRL. We propose \ouralgo, a general framework that can be applied to any dyna-style MBRL method. \ouralgo utilizes Uncertainty-aware Policy-Guided MPC phase to predict the cumulative uncertainty of future steps and symmetrically uses this uncertainty as a penalty or bonus to select actions for conservative model rollouts or optimistic environment exploration. In this way, \ouralgo can avoid model uncertain areas before model rollouts to minimize the impact of model error, while also exploring high-reward model-uncertain areas in the environment to expand the model and reduce model error. Experiments on a range of continuous control tasks demonstrates the effectiveness of our method. One drawback of \ouralgo is that MPC can lead to additional computational time and we provide a detailed computational time consumption in Appendix~\ref{app: exp_cost}. We can improve computational efficiency by parallelizing planning, which we leave for future work.

==> exp/MPCRL_ant.tex <==
% This file was created with tikzplotlib v0.10.1.
\begin{tikzpicture}

\definecolor{darkgray176}{RGB}{176,176,176}
\definecolor{green}{RGB}{0,128,0}

\begin{axis}[
height=9cm, % 修改这里以调整图像高度
width=12cm, % 修改这里以调整图像宽度
ticklabel style={font=\huge},
tick align=outside,
tick pos=left,
title={\Huge\ttfamily{Ant}},
x grid style={darkgray176},
xlabel={\Huge\ttfamily{Steps}},
xmajorgrids,
xmin=-0.7, xmax=14.7,
xtick style={color=black},
xtick={0,3.5,7,10.5,14},
xticklabels={0k,40k,80k,120k,150k},
y grid style={darkgray176},
ylabel={\Huge\ttfamily{Returns}},
ymajorgrids,
ymin=371.998595798074, ymax=5623.25761166765,
ytick style={color=black}
]
\path [draw=red, fill=red, opacity=0.2]
(axis cs:0,692.591221208636)
--(axis cs:0,658.128349329256)
--(axis cs:1,770.978258084543)
--(axis cs:2,1048.53675704539)
--(axis cs:3,1831.63751421671)
--(axis cs:4,1725.72069892719)
--(axis cs:5,1978.63228253525)
--(axis cs:6,2276.40626747808)
--(axis cs:7,3038.45934805091)
--(axis cs:8,3593.59947212808)
--(axis cs:9,4059.54866414824)
--(axis cs:10,4097.95939447887)
--(axis cs:11,4696.77108618562)
--(axis cs:12,4434.57173667975)
--(axis cs:13,5001.05859675084)
--(axis cs:14,5251.5472616735)
--(axis cs:14,5384.56402003721)
--(axis cs:14,5384.56402003721)
--(axis cs:13,5168.13702539828)
--(axis cs:12,4981.70620078772)
--(axis cs:11,4898.53849931712)
--(axis cs:10,4444.87827340848)
--(axis cs:9,4288.66637664174)
--(axis cs:8,3814.2222137736)
--(axis cs:7,3214.35620839773)
--(axis cs:6,2581.89669966912)
--(axis cs:5,2284.87767463288)
--(axis cs:4,1899.63304688971)
--(axis cs:3,1908.93604299845)
--(axis cs:2,1238.71223056085)
--(axis cs:1,792.372471639957)
--(axis cs:0,692.591221208636)
--cycle;

\path [draw=blue, fill=blue, opacity=0.2]
(axis cs:0,663.566974222681)
--(axis cs:0,610.692187428509)
--(axis cs:1,730.461235854197)
--(axis cs:2,916.569245586056)
--(axis cs:3,1102.71875158402)
--(axis cs:4,1620.34946086939)
--(axis cs:5,1463.08404370101)
--(axis cs:6,1805.5908361617)
--(axis cs:7,1861.11842778693)
--(axis cs:8,1794.7189357846)
--(axis cs:9,3001.56860070208)
--(axis cs:10,2673.30453316052)
--(axis cs:11,2743.90179382925)
--(axis cs:12,3048.86626788638)
--(axis cs:13,3488.04764131388)
--(axis cs:14,3253.70989059012)
--(axis cs:14,4795.37328985415)
--(axis cs:14,4795.37328985415)
--(axis cs:13,3934.2991055)
--(axis cs:12,3441.86862685764)
--(axis cs:11,3192.09117916371)
--(axis cs:10,2993.53909570857)
--(axis cs:9,3368.56031937236)
--(axis cs:8,2465.09247303391)
--(axis cs:7,2187.25610500053)
--(axis cs:6,2200.13936727082)
--(axis cs:5,1804.21719390274)
--(axis cs:4,1715.79130776267)
--(axis cs:3,1447.52234294108)
--(axis cs:2,976.765525038416)
--(axis cs:1,779.140959246656)
--(axis cs:0,663.566974222681)
--cycle;

\path [draw=green, fill=green, opacity=0.2]
(axis cs:0,766.706265203295)
--(axis cs:0,746.39532310811)
--(axis cs:1,866.044041027989)
--(axis cs:2,860.644245105421)
--(axis cs:3,1040.79116833682)
--(axis cs:4,1326.87056058328)
--(axis cs:5,1251.64184840135)
--(axis cs:6,1464.13770839206)
--(axis cs:7,1683.09989181747)
--(axis cs:8,1910.77372957263)
--(axis cs:9,1939.67397058076)
--(axis cs:10,1850.24222907405)
--(axis cs:11,1878.84283583555)
--(axis cs:12,2167.22808314977)
--(axis cs:13,2314.86757396906)
--(axis cs:14,2030.1707075448)
--(axis cs:14,2284.87497873571)
--(axis cs:14,2284.87497873571)
--(axis cs:13,2535.15339713995)
--(axis cs:12,2325.30908529115)
--(axis cs:11,2208.41468274054)
--(axis cs:10,2190.06526683666)
--(axis cs:9,2127.21943431597)
--(axis cs:8,2012.02689006184)
--(axis cs:7,1912.58305893742)
--(axis cs:6,1518.22755674177)
--(axis cs:5,1519.60491492207)
--(axis cs:4,1405.89095228153)
--(axis cs:3,1093.03333754351)
--(axis cs:2,889.945310447528)
--(axis cs:1,884.745820722514)
--(axis cs:0,766.706265203295)
--cycle;

\addplot [line width=3pt, red]
table {%
0 674.295652671039
1 780.961184948286
2 1145.01057146238
3 1867.57504109782
4 1795.9819896385
5 2143.20181650406
6 2428.45259113349
7 3132.92076875019
8 3701.35422825756
9 4164.41119608486
10 4275.50371933822
11 4789.60070623224
12 4693.28355559781
13 5081.97935640705
14 5320.07362074275
};
\addplot [line width=3pt, blue]
table {%
0 639.280255611306
1 754.956201966303
2 944.179747062244
3 1266.76805323293
4 1666.87298703545
5 1636.02825042632
6 1988.23997130478
7 2032.86799625067
8 2100.9183741399
9 3190.50365834443
10 2839.44324712066
11 2960.59579914362
12 3251.97061438633
13 3714.77754053747
14 4078.13289983384
};
\addplot [line width=3pt, green]
table {%
0 757.127078265363
1 875.347268204403
2 875.52042466792
3 1067.56071754889
4 1364.0859366385
5 1386.52260395101
6 1492.89181423783
7 1801.69235261806
8 1958.55247504172
9 2024.68601726247
10 2023.04331272119
11 2048.33199386035
12 2237.07504842326
13 2423.92147575603
14 2166.77722594194
};
\end{axis}

\end{tikzpicture}


==> exp/MPCRL_hopper.tex <==
% This file was created with tikzplotlib v0.10.1.
\begin{tikzpicture}

\definecolor{darkgray176}{RGB}{176,176,176}
\definecolor{green}{RGB}{0,128,0}

\begin{axis}[
height=9cm, % 修改这里以调整图像高度
width=12cm, % 修改这里以调整图像宽度
ticklabel style={font=\huge},
tick align=outside,
tick pos=left,
title={\Huge\ttfamily{Hopper}},
x grid style={darkgray176},
xlabel={\Huge\ttfamily{Steps}},
xmajorgrids,
xmin=-0.3, xmax=6.3,
xtick style={color=black},
xtick={0,3,6},
xticklabels={0k,35k,70k},
y grid style={darkgray176},
ylabel={\Huge\ttfamily{Returns}},
ymajorgrids,
ymin=144.580606432391, ymax=3470.04279476522,
ytick style={color=black}
]
\path [draw=red, fill=red, opacity=0.2]
(axis cs:0,365.567679188201)
--(axis cs:0,346.727899255213)
--(axis cs:1,901.230755166124)
--(axis cs:2,1669.13501022359)
--(axis cs:3,2876.1691182433)
--(axis cs:4,2815.95074298149)
--(axis cs:5,3261.88534001267)
--(axis cs:6,3143.51192904929)
--(axis cs:6,3285.44937389548)
--(axis cs:6,3285.44937389548)
--(axis cs:5,3318.88542256827)
--(axis cs:4,3002.88078634001)
--(axis cs:3,2934.94403216566)
--(axis cs:2,2292.66134074338)
--(axis cs:1,1039.94161191779)
--(axis cs:0,365.567679188201)
--cycle;

\path [draw=blue, fill=blue, opacity=0.2]
(axis cs:0,366.336978725382)
--(axis cs:0,299.419810780388)
--(axis cs:1,480.758676042776)
--(axis cs:2,765.246412059402)
--(axis cs:3,1214.88250874692)
--(axis cs:4,1928.69435733309)
--(axis cs:5,1664.26207815606)
--(axis cs:6,2116.45572286922)
--(axis cs:6,2637.15630848569)
--(axis cs:6,2637.15630848569)
--(axis cs:5,2473.92917302845)
--(axis cs:4,2490.26645342206)
--(axis cs:3,1385.66498512094)
--(axis cs:2,913.930206795344)
--(axis cs:1,575.867587434577)
--(axis cs:0,366.336978725382)
--cycle;

\path [draw=green, fill=green, opacity=0.2]
(axis cs:0,337.944920769013)
--(axis cs:0,295.737978629338)
--(axis cs:1,401.478937662388)
--(axis cs:2,588.502910591715)
--(axis cs:3,922.989783387082)
--(axis cs:4,1460.94699614267)
--(axis cs:5,2189.92625174111)
--(axis cs:6,2722.58656800557)
--(axis cs:6,2896.06704307374)
--(axis cs:6,2896.06704307374)
--(axis cs:5,2530.95910908769)
--(axis cs:4,1753.48907639021)
--(axis cs:3,1643.21796651546)
--(axis cs:2,934.662066879705)
--(axis cs:1,461.446569274235)
--(axis cs:0,337.944920769013)
--cycle;

\addplot [line width=3pt, red]
table {%
0 355.949232982477
1 971.212211756104
2 1987.07829798727
3 2902.5378280179
4 2909.32786317425
5 3290.23243870997
6 3215.13890283888
};
\addplot [line width=3pt, blue]
table {%
0 332.945601480507
1 529.044546265673
2 840.567034070348
3 1299.02192763285
4 2210.29980674159
5 2055.219069439
6 2384.86525137626
};
\addplot [line width=3pt, green]
table {%
0 317.379541416445
1 429.347013913468
2 741.701860555188
3 1253.37078577725
4 1606.92807455987
5 2353.11936559839
6 2805.44735584362
};
\end{axis}

\end{tikzpicture}


==> exp/MPCRL_humanoid.tex <==
% This file was created with tikzplotlib v0.10.1.
\begin{tikzpicture}

\definecolor{darkgray176}{RGB}{176,176,176}
\definecolor{green}{RGB}{0,128,0}

\begin{axis}[
height=9cm, % 修改这里以调整图像高度
width=12cm, % 修改这里以调整图像宽度
ticklabel style={font=\huge},
tick align=outside,
tick pos=left,
title={\Huge\ttfamily{Humanoid}},
x grid style={darkgray176},
xlabel={\Huge\ttfamily{Steps}},
xmajorgrids,
xmin=-0.7, xmax=14.7,
xtick style={color=black},
xtick={0,3.5,7,10.5,14},
xticklabels={0k,40k,80k,120k,150k},
y grid style={darkgray176},
ylabel={\Huge\ttfamily{Returns}},
ymajorgrids,
ymin=5.01060170855698, ymax=5971.39816105348,
ytick style={color=black}
]
\path [draw=red, fill=red, opacity=0.2]
(axis cs:0,348.503188367891)
--(axis cs:0,334.599231665549)
--(axis cs:1,447.615281949433)
--(axis cs:2,440.183913739552)
--(axis cs:3,525.008031752409)
--(axis cs:4,574.845830302604)
--(axis cs:5,651.481070104071)
--(axis cs:6,730.686186192819)
--(axis cs:7,1603.09098257894)
--(axis cs:8,2214.47462986219)
--(axis cs:9,2750.49748481753)
--(axis cs:10,3075.83048204405)
--(axis cs:11,2634.75872400309)
--(axis cs:12,3177.33062840781)
--(axis cs:13,4605.55536427321)
--(axis cs:14,4978.18153146748)
--(axis cs:14,5700.1987265378)
--(axis cs:14,5700.1987265378)
--(axis cs:13,4862.10092447618)
--(axis cs:12,3773.53122743321)
--(axis cs:11,3268.96647794755)
--(axis cs:10,3233.65247356624)
--(axis cs:9,3123.67279637704)
--(axis cs:8,2612.008140677)
--(axis cs:7,2428.36638873609)
--(axis cs:6,822.921942505658)
--(axis cs:5,726.396992746175)
--(axis cs:4,631.106030798392)
--(axis cs:3,557.240732586774)
--(axis cs:2,456.689710071167)
--(axis cs:1,462.10768959425)
--(axis cs:0,348.503188367891)
--cycle;

\path [draw=blue, fill=blue, opacity=0.2]
(axis cs:0,294.694314924291)
--(axis cs:0,279.191557643678)
--(axis cs:1,359.317587894026)
--(axis cs:2,415.601498726813)
--(axis cs:3,473.119698221123)
--(axis cs:4,522.781589297185)
--(axis cs:5,531.79258991189)
--(axis cs:6,600.70298891609)
--(axis cs:7,734.039691520531)
--(axis cs:8,1044.28136944488)
--(axis cs:9,1305.13303872761)
--(axis cs:10,1348.11054227148)
--(axis cs:11,1663.57847493008)
--(axis cs:12,2576.31908550684)
--(axis cs:13,2937.94490200486)
--(axis cs:14,3644.13216915692)
--(axis cs:14,5054.11856439076)
--(axis cs:14,5054.11856439076)
--(axis cs:13,4642.60964612222)
--(axis cs:12,3812.35491681892)
--(axis cs:11,3242.09899270862)
--(axis cs:10,3262.90956836147)
--(axis cs:9,2611.58531741309)
--(axis cs:8,2300.74818386951)
--(axis cs:7,897.544667683899)
--(axis cs:6,807.212319665532)
--(axis cs:5,599.06395453726)
--(axis cs:4,541.120584074017)
--(axis cs:3,485.766406017064)
--(axis cs:2,435.156634800743)
--(axis cs:1,385.910880889813)
--(axis cs:0,294.694314924291)
--cycle;

\path [draw=green, fill=green, opacity=0.2]
(axis cs:0,313.333403748333)
--(axis cs:0,276.210036224235)
--(axis cs:1,360.599588367666)
--(axis cs:2,418.409396085367)
--(axis cs:3,452.039617762471)
--(axis cs:4,538.275022488806)
--(axis cs:5,524.137060692484)
--(axis cs:6,598.320852641474)
--(axis cs:7,714.908026731789)
--(axis cs:8,565.288973962477)
--(axis cs:9,751.404332232285)
--(axis cs:10,847.220867033786)
--(axis cs:11,1012.1485051043)
--(axis cs:12,1199.54215976721)
--(axis cs:13,1230.25198763004)
--(axis cs:14,1730.99657485406)
--(axis cs:14,2742.61275178485)
--(axis cs:14,2742.61275178485)
--(axis cs:13,1715.78674186417)
--(axis cs:12,1592.57858305173)
--(axis cs:11,1182.3914467036)
--(axis cs:10,932.72257956676)
--(axis cs:9,878.03328023717)
--(axis cs:8,678.851618662463)
--(axis cs:7,739.935219738888)
--(axis cs:6,601.115785585308)
--(axis cs:5,563.38520715076)
--(axis cs:4,549.255432542553)
--(axis cs:3,466.73798221904)
--(axis cs:2,463.427793271885)
--(axis cs:1,375.618057472171)
--(axis cs:0,313.333403748333)
--cycle;

\addplot [line width=3pt, red]
table {%
0 340.98578114132
1 454.378179772521
2 447.867080983342
3 541.988704149226
4 600.563004456433
5 690.324915662408
6 779.173419891895
7 2017.36364869918
8 2424.0862160305
9 2941.46256839784
10 3155.00882426327
11 2938.73361660411
12 3461.82164308562
13 4731.03658003243
14 5324.09004145826
};
\addplot [line width=3pt, blue]
table {%
0 287.545669582592
1 373.188046254266
2 425.245473071132
3 478.833529885139
4 531.455189082565
5 564.379187225444
6 691.26183767682
7 817.470120309379
8 1614.57235959976
9 1903.55150162003
10 2281.75965298842
11 2414.87546539131
12 3169.20584246024
13 3765.70860089468
14 4366.51446910827
};
\addplot [line width=3pt, green]
table {%
0 293.646558466903
1 368.15848774876
2 440.585568508443
3 459.452456262892
4 543.750314993613
5 542.842728236343
6 599.768650131149
7 727.474820085162
8 621.865048469842
9 814.069453134409
10 889.295030236898
11 1096.32457732202
12 1398.13828928648
13 1459.31412143844
14 2221.97873591038
};
\end{axis}

\end{tikzpicture}


==> exp/MPCRL_walker.tex <==
% This file was created with tikzplotlib v0.10.1.
\begin{tikzpicture}

\definecolor{darkgray176}{RGB}{176,176,176}
\definecolor{green}{RGB}{0,128,0}
\definecolor{lightgray204}{RGB}{204,204,204}

\begin{axis}[
height=9cm, % 修改这里以调整图像高度
width=12cm, % 修改这里以调整图像宽度
legend cell align={left},
legend style={
  fill opacity=0.8,
  draw opacity=1,
  text opacity=1,
  at={(0.97,0.03)},
  anchor=south east,
  draw=lightgray204,
  font=\Large\ttfamily
},
ticklabel style={font=\huge},
tick align=outside,
tick pos=left,
title={\Huge\ttfamily{Walker}},
x grid style={darkgray176},
xlabel={\Huge\ttfamily{Steps}},
xmajorgrids,
xmin=-0.7, xmax=14.7,
xtick style={color=black},
xtick={0,3.5,7,10.5,14},
xticklabels={0k,40k,80k,120k,150k},
y grid style={darkgray176},
ylabel={\Huge\ttfamily{Returns}},
ymajorgrids,
ymin=-2.17301777072649, ymax=4927.39246230607,
ytick style={color=black}
]
\path [draw=red, fill=red, opacity=0.2]
(axis cs:0,399.620701981819)
--(axis cs:0,348.864729171443)
--(axis cs:1,471.74714905198)
--(axis cs:2,633.613900795428)
--(axis cs:3,1322.10728798529)
--(axis cs:4,1942.24716657106)
--(axis cs:5,2609.66645060628)
--(axis cs:6,2864.35458088093)
--(axis cs:7,3426.26102943363)
--(axis cs:8,3713.80531018044)
--(axis cs:9,3857.15419070206)
--(axis cs:10,4082.66948314944)
--(axis cs:11,4034.68327916265)
--(axis cs:12,4225.21629357885)
--(axis cs:13,4192.03047121243)
--(axis cs:14,4194.10923448293)
--(axis cs:14,4703.32130412076)
--(axis cs:14,4703.32130412076)
--(axis cs:13,4633.34448880033)
--(axis cs:12,4699.13329716583)
--(axis cs:11,4413.98448680828)
--(axis cs:10,4457.51872854862)
--(axis cs:9,4352.55680400534)
--(axis cs:8,4321.47489313528)
--(axis cs:7,4174.38560830534)
--(axis cs:6,3708.30967978315)
--(axis cs:5,3394.93036168108)
--(axis cs:4,2520.36185784767)
--(axis cs:3,1707.75526768342)
--(axis cs:2,743.216011779856)
--(axis cs:1,619.699395776713)
--(axis cs:0,399.620701981819)
--cycle;

\path [draw=blue, fill=blue, opacity=0.2]
(axis cs:0,326.475155746736)
--(axis cs:0,277.415968323852)
--(axis cs:1,499.192658402397)
--(axis cs:2,817.947669932831)
--(axis cs:3,667.143910975686)
--(axis cs:4,871.925978355428)
--(axis cs:5,1135.76834893467)
--(axis cs:6,1922.11542468971)
--(axis cs:7,2066.18654762018)
--(axis cs:8,2934.42951081693)
--(axis cs:9,2818.57896101266)
--(axis cs:10,3028.55961781651)
--(axis cs:11,3234.49101045219)
--(axis cs:12,3527.44229797741)
--(axis cs:13,3967.66438184426)
--(axis cs:14,3580.36269713952)
--(axis cs:14,3970.85808884487)
--(axis cs:14,3970.85808884487)
--(axis cs:13,4190.38351021724)
--(axis cs:12,4043.61322240043)
--(axis cs:11,3791.62457162195)
--(axis cs:10,3941.4635418315)
--(axis cs:9,3551.17762568592)
--(axis cs:8,4007.81420170847)
--(axis cs:7,3008.30392658826)
--(axis cs:6,2477.92617159108)
--(axis cs:5,1518.45548490914)
--(axis cs:4,1017.82866529182)
--(axis cs:3,812.075590229456)
--(axis cs:2,1122.00256177844)
--(axis cs:1,589.243628286744)
--(axis cs:0,326.475155746736)
--cycle;

\path [draw=green, fill=green, opacity=0.2]
(axis cs:0,252.634482855558)
--(axis cs:0,221.898140414582)
--(axis cs:1,424.502995708018)
--(axis cs:2,484.616998298876)
--(axis cs:3,566.165632774203)
--(axis cs:4,850.182134818752)
--(axis cs:5,1330.68271208137)
--(axis cs:6,1853.8772168305)
--(axis cs:7,2691.15032318578)
--(axis cs:8,2908.65637174292)
--(axis cs:9,2742.70386888535)
--(axis cs:10,3558.34313446112)
--(axis cs:11,3372.86502074924)
--(axis cs:12,3681.31294738329)
--(axis cs:13,3744.63275249585)
--(axis cs:14,3899.24324312945)
--(axis cs:14,4114.56646405604)
--(axis cs:14,4114.56646405604)
--(axis cs:13,4094.70543789034)
--(axis cs:12,3995.41498019351)
--(axis cs:11,3954.27066483566)
--(axis cs:10,3824.67762871517)
--(axis cs:9,3332.62911183771)
--(axis cs:8,3034.58675955724)
--(axis cs:7,3001.50283250373)
--(axis cs:6,2409.85419999517)
--(axis cs:5,1848.08616866287)
--(axis cs:4,955.027896985465)
--(axis cs:3,682.410014061872)
--(axis cs:2,579.64798797905)
--(axis cs:1,492.690476692922)
--(axis cs:0,252.634482855558)
--cycle;

\addplot [line width=3pt, red]
table {%
0 374.532703571514
1 545.570253655694
2 688.961663694537
3 1510.25392313513
4 2231.71855552911
5 3001.62773370753
6 3297.23044678807
7 3786.51006355758
8 4014.1794018168
9 4107.66499508486
10 4267.86136206808
11 4208.09482389694
12 4464.62696897541
13 4412.10254112788
14 4448.01270774961
};
\addlegendentry{CO-Planner-MBPO}
\addplot [line width=3pt, blue]
table {%
0 301.216738499863
1 545.201301747185
2 965.602888352284
3 737.061731914987
4 940.548457649332
5 1307.42911848735
6 2188.89617561749
7 2551.53136285306
8 3476.23776995635
9 3213.36908648188
10 3492.295916398
11 3494.69806649255
12 3794.40185883108
13 4079.08572384281
14 3765.16019254064
};
\addlegendentry{P2P-MPC}
\addplot [line width=3pt, green]
table {%
0 237.384205011841
1 458.827388866781
2 530.430820605997
3 624.480507653377
4 903.339187826515
5 1571.59379624329
6 2128.95010681862
7 2845.53788638808
8 2969.21629947685
9 3027.410495376
10 3682.16352508827
11 3686.90642234443
12 3847.25871233141
13 3929.68680839437
14 4002.34950701241
};
\addlegendentry{MBPO}
\end{axis}

\end{tikzpicture}


==> exp/ablation_study/walker-run_exploit_rate.tex <==
% This file was created with tikzplotlib v0.10.1.
\begin{tikzpicture}

\definecolor{darkgray176}{RGB}{176,176,176}
\definecolor{darkorange}{RGB}{255,140,0}
\definecolor{green}{RGB}{0,128,0}
\definecolor{lightgray204}{RGB}{204,204,204}
\definecolor{purple}{RGB}{128,0,128}

\begin{axis}[
legend cell align={left},
legend style={
  fill opacity=0.8,
  draw opacity=1,
  text opacity=1,
  at={(0.03,0.97)},
  anchor=north west,
  draw=lightgray204
},
tick align=outside,
tick pos=left,
title={Walker-run},
x grid style={darkgray176},
xmajorgrids,
xmin=-0.95, xmax=19.95,
xtick style={color=black},
y grid style={darkgray176},
ymajorgrids,
ymin=-9.77976631933335, ymax=610.530421344321,
ytick style={color=black}
]
\path [draw=green, fill=green, opacity=0.2]
(axis cs:0,26.5452033507545)
--(axis cs:0,25.4768274251621)
--(axis cs:1,44.3168630840182)
--(axis cs:2,115.664663069547)
--(axis cs:3,159.361481275755)
--(axis cs:4,172.924381270753)
--(axis cs:5,199.898983259298)
--(axis cs:6,243.717048512285)
--(axis cs:7,283.340376011778)
--(axis cs:8,303.445627075423)
--(axis cs:9,331.68344169084)
--(axis cs:10,350.384749104618)
--(axis cs:11,371.473209110371)
--(axis cs:12,384.980071600884)
--(axis cs:13,401.334943161185)
--(axis cs:14,411.697996936465)
--(axis cs:15,420.134588751592)
--(axis cs:16,430.267473755227)
--(axis cs:17,433.923250751347)
--(axis cs:18,441.645007375674)
--(axis cs:19,447.432527284637)
--(axis cs:19,485.376314875218)
--(axis cs:19,485.376314875218)
--(axis cs:18,479.363705507009)
--(axis cs:17,478.753955590371)
--(axis cs:16,478.050136469735)
--(axis cs:15,472.733490392504)
--(axis cs:14,468.650045974569)
--(axis cs:13,460.071436958599)
--(axis cs:12,436.002085460338)
--(axis cs:11,422.140610163673)
--(axis cs:10,405.97259234051)
--(axis cs:9,385.600721982415)
--(axis cs:8,359.256932278364)
--(axis cs:7,335.475679267264)
--(axis cs:6,302.373569494713)
--(axis cs:5,248.296447619553)
--(axis cs:4,218.426043161926)
--(axis cs:3,168.247883131599)
--(axis cs:2,130.282293838835)
--(axis cs:1,56.0607325557334)
--(axis cs:0,26.5452033507545)
--cycle;

\path [draw=red, fill=red, opacity=0.2]
(axis cs:0,24.4621103755634)
--(axis cs:0,23.4814486801795)
--(axis cs:1,37.1946824077598)
--(axis cs:2,88.4796951664913)
--(axis cs:3,151.779237101436)
--(axis cs:4,174.267564925924)
--(axis cs:5,227.958971827983)
--(axis cs:6,283.855964649777)
--(axis cs:7,344.536653265396)
--(axis cs:8,380.950236625026)
--(axis cs:9,413.31341900415)
--(axis cs:10,439.792435928298)
--(axis cs:11,452.924459970176)
--(axis cs:12,466.8002914815)
--(axis cs:13,485.734243449711)
--(axis cs:14,488.214765970411)
--(axis cs:15,501.380869456998)
--(axis cs:16,501.607732237932)
--(axis cs:17,502.92662936316)
--(axis cs:18,516.985989331634)
--(axis cs:19,522.269556982961)
--(axis cs:19,582.334503723246)
--(axis cs:19,582.334503723246)
--(axis cs:18,578.878504033989)
--(axis cs:17,558.973241082656)
--(axis cs:16,561.065439204361)
--(axis cs:15,560.851456610611)
--(axis cs:14,541.498997758081)
--(axis cs:13,538.045298408633)
--(axis cs:12,524.71781918778)
--(axis cs:11,511.670906579885)
--(axis cs:10,501.862907680394)
--(axis cs:9,475.488188424806)
--(axis cs:8,451.284398263622)
--(axis cs:7,416.391434100144)
--(axis cs:6,350.625612736763)
--(axis cs:5,275.618013292747)
--(axis cs:4,183.039909500712)
--(axis cs:3,157.277396885758)
--(axis cs:2,115.859711251082)
--(axis cs:1,51.0806183558788)
--(axis cs:0,24.4621103755634)
--cycle;

\path [draw=blue, fill=blue, opacity=0.2]
(axis cs:0,25.9446400635925)
--(axis cs:0,23.1402101611456)
--(axis cs:1,53.5406262582577)
--(axis cs:2,116.752168458276)
--(axis cs:3,157.058229721255)
--(axis cs:4,192.463672235872)
--(axis cs:5,233.414258246093)
--(axis cs:6,265.264469866407)
--(axis cs:7,298.22183857763)
--(axis cs:8,360.731265823961)
--(axis cs:9,382.532143195366)
--(axis cs:10,404.059303506018)
--(axis cs:11,422.151652469047)
--(axis cs:12,449.034704305926)
--(axis cs:13,470.270780371057)
--(axis cs:14,475.670107850016)
--(axis cs:15,496.977294056217)
--(axis cs:16,501.46978493816)
--(axis cs:17,508.518344583786)
--(axis cs:18,520.304989895678)
--(axis cs:19,515.026554039865)
--(axis cs:19,580.768143998712)
--(axis cs:19,580.768143998712)
--(axis cs:18,579.233038895292)
--(axis cs:17,570.167083587522)
--(axis cs:16,561.677145851706)
--(axis cs:15,553.458879939961)
--(axis cs:14,535.714084957068)
--(axis cs:13,536.380398360176)
--(axis cs:12,514.581023570276)
--(axis cs:11,490.76270982818)
--(axis cs:10,476.71121048998)
--(axis cs:9,457.006347635526)
--(axis cs:8,424.629557241462)
--(axis cs:7,383.999580578359)
--(axis cs:6,349.159469683094)
--(axis cs:5,313.6832589886)
--(axis cs:4,254.77948367527)
--(axis cs:3,170.698992834713)
--(axis cs:2,136.77223536329)
--(axis cs:1,62.0237232170378)
--(axis cs:0,25.9446400635925)
--cycle;

\path [draw=purple, fill=purple, opacity=0.2]
(axis cs:0,25.1779747184794)
--(axis cs:0,22.993365779668)
--(axis cs:1,46.9660523847384)
--(axis cs:2,102.861467807961)
--(axis cs:3,132.914847245707)
--(axis cs:4,157.611608901874)
--(axis cs:5,181.732766515413)
--(axis cs:6,211.034044509804)
--(axis cs:7,266.922817025268)
--(axis cs:8,305.160606232143)
--(axis cs:9,333.591080289169)
--(axis cs:10,356.020781309194)
--(axis cs:11,372.989744336001)
--(axis cs:12,390.109468730624)
--(axis cs:13,415.234472382072)
--(axis cs:14,418.15964782114)
--(axis cs:15,434.537241553497)
--(axis cs:16,446.109498404925)
--(axis cs:17,455.582936772142)
--(axis cs:18,467.595809346695)
--(axis cs:19,476.960683872088)
--(axis cs:19,503.169226779349)
--(axis cs:19,503.169226779349)
--(axis cs:18,496.12627088398)
--(axis cs:17,484.848129794229)
--(axis cs:16,478.972352626744)
--(axis cs:15,476.072866302087)
--(axis cs:14,461.743740494639)
--(axis cs:13,461.655426308956)
--(axis cs:12,439.939896681181)
--(axis cs:11,422.656241365311)
--(axis cs:10,405.718366250296)
--(axis cs:9,380.364696134927)
--(axis cs:8,351.806717797033)
--(axis cs:7,313.627704740364)
--(axis cs:6,253.426860290945)
--(axis cs:5,213.679265488192)
--(axis cs:4,173.182495151474)
--(axis cs:3,156.203579066536)
--(axis cs:2,130.505364491999)
--(axis cs:1,58.5600137065701)
--(axis cs:0,25.1779747184794)
--cycle;

\path [draw=darkorange, fill=darkorange, opacity=0.2]
(axis cs:0,19.7403534887727)
--(axis cs:0,18.4161513017419)
--(axis cs:1,52.2966960016659)
--(axis cs:2,101.74122166323)
--(axis cs:3,155.425484815178)
--(axis cs:4,152.585990832686)
--(axis cs:5,172.494413696223)
--(axis cs:6,221.413039187709)
--(axis cs:7,264.549480908303)
--(axis cs:8,290.829366880499)
--(axis cs:9,326.755273722006)
--(axis cs:10,349.315834452743)
--(axis cs:11,362.741234954762)
--(axis cs:12,397.894609450579)
--(axis cs:13,421.056606256208)
--(axis cs:14,431.299652356309)
--(axis cs:15,445.001153397542)
--(axis cs:16,452.540925703454)
--(axis cs:17,453.01241276329)
--(axis cs:18,460.571459350991)
--(axis cs:19,470.639882731182)
--(axis cs:19,499.051332385624)
--(axis cs:19,499.051332385624)
--(axis cs:18,488.642887152023)
--(axis cs:17,477.193942242617)
--(axis cs:16,479.687787341582)
--(axis cs:15,469.867996142778)
--(axis cs:14,454.653252423744)
--(axis cs:13,445.151527233273)
--(axis cs:12,420.059302824111)
--(axis cs:11,393.759522894819)
--(axis cs:10,388.360003330748)
--(axis cs:9,356.851900090915)
--(axis cs:8,318.438306540999)
--(axis cs:7,284.472670199022)
--(axis cs:6,236.454949273388)
--(axis cs:5,180.783809823694)
--(axis cs:4,161.466386204237)
--(axis cs:3,160.842039095332)
--(axis cs:2,132.373467005841)
--(axis cs:1,67.0925610847476)
--(axis cs:0,19.7403534887727)
--cycle;

\addplot [very thick, green]
table {%
0 25.9807576141283
1 50.3333474834778
2 122.123772921227
3 163.762335033537
4 194.644723254572
5 223.381269730325
6 272.199374023475
7 306.978056157191
8 330.141817388583
9 357.256869656539
10 378.31494543652
11 395.524027846495
12 409.750398639487
13 431.5019102181
14 439.469335111241
15 446.955902025436
16 454.899199431928
17 457.684572255525
18 461.634129203773
19 466.8635318766
};
\addlegendentry{Exploit=4}
\addplot [very thick, red]
table {%
0 23.9795189038959
1 43.9556256195821
2 100.544647252064
3 154.609543746881
4 178.415615487468
5 253.41472236109
6 317.018663715009
7 380.124442556598
8 414.92981286091
9 445.331930182894
10 467.795856453344
11 481.821669529288
12 494.26490292329
13 509.948502654855
14 513.796190996439
15 529.989513271107
16 530.129060972806
17 531.316229238717
18 544.788611700525
19 551.625437275081
};
\addlegendentry{Exploit=2}
\addplot [very thick, blue]
table {%
0 24.5700106095036
1 57.4385430565171
2 126.670757031838
3 163.795643756034
4 221.030743237023
5 271.39470014345
6 306.415463755475
7 339.558928350431
8 393.697993248729
9 419.525243544073
10 438.620549918165
11 456.302854408715
12 479.242463419211
13 500.555025592624
14 504.37653170877
15 523.668324046075
16 530.278720647094
17 538.764002094299
18 549.05141482575
19 547.003183043439
};
\addlegendentry{Exploit=1}
\addplot [very thick, purple]
table {%
0 24.0504514243473
1 52.7858579883958
2 117.434144129845
3 145.367953126818
4 165.811278668078
5 196.641217187722
6 231.665957746806
7 288.600485435076
8 328.367894686634
9 357.843161502237
10 380.605902465173
11 398.97014334293
12 415.144895189323
13 440.009885653123
14 442.297071759333
15 456.897795463942
16 463.405987089243
17 470.861569405342
18 481.977122339137
19 489.777260836816
};
\addlegendentry{Exploit=0.5}
\addplot [very thick, darkorange]
table {%
0 19.1233619551996
1 59.4315382358616
2 117.076752163985
3 158.403216328628
4 157.507467610618
5 176.673825009742
6 229.343690617849
7 273.89763499719
8 304.674817369149
9 341.863892792578
10 368.837557327768
11 378.319116007318
12 408.98112603768
13 432.044107232248
14 443.874017049792
15 458.019666785549
16 466.157864249473
17 465.8827250276
18 475.761479821276
19 485.167140763462
};
\addlegendentry{Exploit=0.1}
\end{axis}

\end{tikzpicture}


==> exp/ablation_study/walker-run_explore_rate.tex <==
% This file was created with tikzplotlib v0.10.1.
\begin{tikzpicture}

\definecolor{darkgray176}{RGB}{176,176,176}
\definecolor{darkorange}{RGB}{255,140,0}
\definecolor{green}{RGB}{0,128,0}
\definecolor{lightgray204}{RGB}{204,204,204}
\definecolor{purple}{RGB}{128,0,128}

\begin{axis}[
legend cell align={left},
legend style={
  fill opacity=0.8,
  draw opacity=1,
  text opacity=1,
  at={(0.03,0.97)},
  anchor=north west,
  draw=lightgray204
},
tick align=outside,
tick pos=left,
title={Walker-run},
x grid style={darkgray176},
xmajorgrids,
xmin=-0.95, xmax=19.95,
xtick style={color=black},
y grid style={darkgray176},
ymajorgrids,
ymin=-7.73321263768682, ymax=608.885784413689,
ytick style={color=black}
]
\path [draw=blue, fill=blue, opacity=0.2]
(axis cs:0,28.2438873645131)
--(axis cs:0,26.2075023257554)
--(axis cs:1,56.1728931987876)
--(axis cs:2,124.449938056064)
--(axis cs:3,159.224169226722)
--(axis cs:4,170.07767300588)
--(axis cs:5,212.446429413212)
--(axis cs:6,258.405760214636)
--(axis cs:7,291.360733873542)
--(axis cs:8,340.777970244154)
--(axis cs:9,375.508060158286)
--(axis cs:10,388.307249617674)
--(axis cs:11,416.861392505369)
--(axis cs:12,436.746908556825)
--(axis cs:13,461.834989884621)
--(axis cs:14,464.841190148157)
--(axis cs:15,481.147806951943)
--(axis cs:16,488.29256423701)
--(axis cs:17,494.321699674502)
--(axis cs:18,504.811667879845)
--(axis cs:19,515.107802604523)
--(axis cs:19,540.117823601885)
--(axis cs:19,540.117823601885)
--(axis cs:18,531.198433433881)
--(axis cs:17,515.378620895456)
--(axis cs:16,513.036500939423)
--(axis cs:15,501.126805628041)
--(axis cs:14,483.324470886177)
--(axis cs:13,479.386246758016)
--(axis cs:12,453.967885436348)
--(axis cs:11,434.273189255648)
--(axis cs:10,412.660127340058)
--(axis cs:9,391.901847426915)
--(axis cs:8,357.793395409736)
--(axis cs:7,314.370147285552)
--(axis cs:6,279.511207119636)
--(axis cs:5,238.283620792586)
--(axis cs:4,183.202631988573)
--(axis cs:3,165.573801420802)
--(axis cs:2,143.217172982935)
--(axis cs:1,73.8265958401135)
--(axis cs:0,28.2438873645131)
--cycle;

\path [draw=green, fill=green, opacity=0.2]
(axis cs:0,22.7396352943575)
--(axis cs:0,20.2949235919212)
--(axis cs:1,50.1578402307532)
--(axis cs:2,111.380805997707)
--(axis cs:3,153.003994108584)
--(axis cs:4,197.607285407491)
--(axis cs:5,246.372176588105)
--(axis cs:6,308.449213513899)
--(axis cs:7,352.946964827947)
--(axis cs:8,378.250335555547)
--(axis cs:9,402.610450141606)
--(axis cs:10,421.661113918393)
--(axis cs:11,435.005587608567)
--(axis cs:12,430.950234679679)
--(axis cs:13,459.602515904141)
--(axis cs:14,467.548492862908)
--(axis cs:15,480.842497388775)
--(axis cs:16,490.219171617668)
--(axis cs:17,485.358793691936)
--(axis cs:18,458.955584610237)
--(axis cs:19,406.183982238766)
--(axis cs:19,513.11904278497)
--(axis cs:19,513.11904278497)
--(axis cs:18,518.860772655573)
--(axis cs:17,520.15019362214)
--(axis cs:16,522.089598781455)
--(axis cs:15,510.025330320152)
--(axis cs:14,495.481368458763)
--(axis cs:13,492.32622753163)
--(axis cs:12,472.570211076151)
--(axis cs:11,475.019271059804)
--(axis cs:10,465.512304266709)
--(axis cs:9,448.010670670222)
--(axis cs:8,427.513265379875)
--(axis cs:7,397.448856187963)
--(axis cs:6,367.295074319465)
--(axis cs:5,321.923745309983)
--(axis cs:4,277.089320906367)
--(axis cs:3,204.984098217699)
--(axis cs:2,133.069225709793)
--(axis cs:1,58.1858223291314)
--(axis cs:0,22.7396352943575)
--cycle;

\path [draw=red, fill=red, opacity=0.2]
(axis cs:0,24.453374617354)
--(axis cs:0,23.4769770231036)
--(axis cs:1,37.331791718186)
--(axis cs:2,88.3047354924283)
--(axis cs:3,151.593610881749)
--(axis cs:4,173.960162828344)
--(axis cs:5,228.080171881818)
--(axis cs:6,282.794874228841)
--(axis cs:7,343.342826936731)
--(axis cs:8,379.559720086959)
--(axis cs:9,413.922174689202)
--(axis cs:10,438.782238479491)
--(axis cs:11,452.307317767251)
--(axis cs:12,464.741001191892)
--(axis cs:13,482.705310218556)
--(axis cs:14,488.577533491886)
--(axis cs:15,502.766771737399)
--(axis cs:16,503.070350082272)
--(axis cs:17,504.90647559965)
--(axis cs:18,515.300026433185)
--(axis cs:19,523.986028823208)
--(axis cs:19,578.929054040344)
--(axis cs:19,578.929054040344)
--(axis cs:18,577.477855048383)
--(axis cs:17,562.829558287402)
--(axis cs:16,558.934383288894)
--(axis cs:15,562.37755865598)
--(axis cs:14,541.577757959795)
--(axis cs:13,538.910564954042)
--(axis cs:12,525.579433444732)
--(axis cs:11,511.876194417463)
--(axis cs:10,498.182391818029)
--(axis cs:9,477.420277779808)
--(axis cs:8,448.132293585278)
--(axis cs:7,417.550576806783)
--(axis cs:6,351.672721478384)
--(axis cs:5,276.606069847449)
--(axis cs:4,182.897843400468)
--(axis cs:3,157.733114682564)
--(axis cs:2,114.269435905592)
--(axis cs:1,50.1718273056835)
--(axis cs:0,24.453374617354)
--cycle;

\path [draw=purple, fill=purple, opacity=0.2]
(axis cs:0,25.3745201291246)
--(axis cs:0,23.3093445338975)
--(axis cs:1,42.6398050594703)
--(axis cs:2,127.292063793137)
--(axis cs:3,175.12248234773)
--(axis cs:4,213.425139738471)
--(axis cs:5,266.865034147265)
--(axis cs:6,305.651687913566)
--(axis cs:7,342.190561841206)
--(axis cs:8,374.339303681892)
--(axis cs:9,404.60798498612)
--(axis cs:10,416.274406041051)
--(axis cs:11,434.211531804904)
--(axis cs:12,455.415712481991)
--(axis cs:13,481.143201978335)
--(axis cs:14,493.690990153706)
--(axis cs:15,506.046367209832)
--(axis cs:16,518.695720630755)
--(axis cs:17,522.025261483926)
--(axis cs:18,534.878992008367)
--(axis cs:19,545.093093450719)
--(axis cs:19,580.857648184081)
--(axis cs:19,580.857648184081)
--(axis cs:18,565.687077539694)
--(axis cs:17,555.898015568542)
--(axis cs:16,551.870352936959)
--(axis cs:15,541.589017901323)
--(axis cs:14,528.235248914161)
--(axis cs:13,523.407624603103)
--(axis cs:12,506.87331594998)
--(axis cs:11,494.844623541372)
--(axis cs:10,479.693025159511)
--(axis cs:9,466.071307240095)
--(axis cs:8,437.805416347704)
--(axis cs:7,415.416562209584)
--(axis cs:6,384.674424855164)
--(axis cs:5,337.874682173689)
--(axis cs:4,294.107373660815)
--(axis cs:3,211.631954698222)
--(axis cs:2,142.170399632247)
--(axis cs:1,48.7067199798525)
--(axis cs:0,25.3745201291246)
--cycle;

\path [draw=darkorange, fill=darkorange, opacity=0.2]
(axis cs:0,27.5013119786416)
--(axis cs:0,24.6091135273065)
--(axis cs:1,52.1658859812075)
--(axis cs:2,112.389965321772)
--(axis cs:3,156.680852205958)
--(axis cs:4,167.729621330486)
--(axis cs:5,180.30438735544)
--(axis cs:6,215.943552660134)
--(axis cs:7,268.03668463734)
--(axis cs:8,334.69055465238)
--(axis cs:9,369.066955260635)
--(axis cs:10,397.706091601495)
--(axis cs:11,414.855652981172)
--(axis cs:12,429.642329671898)
--(axis cs:13,448.669197913966)
--(axis cs:14,451.768838379668)
--(axis cs:15,465.053463222302)
--(axis cs:16,476.852458798655)
--(axis cs:17,483.02255038392)
--(axis cs:18,493.214952564156)
--(axis cs:19,506.507582976537)
--(axis cs:19,522.847736791563)
--(axis cs:19,522.847736791563)
--(axis cs:18,513.828368007728)
--(axis cs:17,501.668850011044)
--(axis cs:16,493.647657036682)
--(axis cs:15,481.415372928654)
--(axis cs:14,471.52277467873)
--(axis cs:13,468.163785365515)
--(axis cs:12,449.890652886819)
--(axis cs:11,433.893839154027)
--(axis cs:10,418.335896167075)
--(axis cs:9,396.746801606452)
--(axis cs:8,366.35490178025)
--(axis cs:7,314.143496534883)
--(axis cs:6,266.939011857841)
--(axis cs:5,229.621130977563)
--(axis cs:4,206.110887696182)
--(axis cs:3,168.032959209)
--(axis cs:2,141.690494216983)
--(axis cs:1,70.079523559872)
--(axis cs:0,27.5013119786416)
--cycle;

\addplot [very thick, blue]
table {%
0 27.2277924581189
1 65.1667120907791
2 134.700162401053
3 162.448324655598
4 175.693137818847
5 224.921910689069
6 268.521650497082
7 302.351017630104
8 349.409329354438
9 383.106730774341
10 400.033369348266
11 425.017740162046
12 445.234921060883
13 470.506321196983
14 473.890824797394
15 491.500607770102
16 501.247224616993
17 505.249772994977
18 518.073052508409
19 528.216569492452
};
\addlegendentry{explore=4}
\addplot [very thick, green]
table {%
0 21.6052965327307
1 54.2383403180969
2 122.236198003596
3 176.793691539374
4 235.087671339363
5 283.766052375008
6 337.620936671219
7 373.796369131899
8 402.917827317674
9 422.723614178671
10 443.104365802115
11 453.732267656526
12 450.730394682105
13 475.936916828583
14 480.70529426115
15 494.392163747415
16 504.264321971513
17 501.477375656223
18 488.751491084124
19 465.811357761965
};
\addlegendentry{explore=2}
\addplot [very thick, red]
table {%
0 23.9749269400612
1 43.7234813350556
2 100.647403020332
3 154.621004030078
4 178.393769233827
5 253.876674650115
6 316.871645900789
7 380.752913468585
8 415.529358544742
9 446.185887249073
10 468.412284570154
11 482.038409574243
12 494.22867398112
13 509.915950282138
14 513.756207288073
15 530.194235958823
16 530.244043761101
17 531.405652604193
18 545.42813567097
19 551.211410365791
};
\addlegendentry{explore=1}
\addplot [very thick, purple]
table {%
0 24.3803285083114
1 45.9556611542583
2 134.275978845406
3 191.75090583928
4 252.360095868196
5 303.659789977055
6 347.970112851894
7 379.599260156576
8 408.313767724882
9 436.209210035865
10 449.268934541296
11 465.017540990757
12 482.312642045447
13 502.553350599837
14 510.437906106069
15 523.393086351263
16 535.118754677626
17 539.408120610565
18 550.753173159143
19 562.26923060421
};
\addlegendentry{explore=0.5}
\addplot [very thick, darkorange]
table {%
0 26.0939961470142
1 60.6939557560582
2 127.106615336379
3 162.393459008669
4 185.135219869119
5 203.838715827133
6 239.605531051505
7 290.297869483041
8 350.351230618322
9 382.294190585044
10 407.476284019383
11 423.851557225815
12 439.108959560018
13 457.939073230314
14 461.375182666196
15 472.732930985529
16 485.115748334739
17 491.931815893397
18 502.747482871055
19 514.374082000523
};
\addlegendentry{explore=0.1}
\end{axis}

\end{tikzpicture}


==> exp/ablation_study/walker-run_ntraj.tex <==
% This file was created with tikzplotlib v0.10.1.
\begin{tikzpicture}

\definecolor{darkgray176}{RGB}{176,176,176}
\definecolor{green}{RGB}{0,128,0}
\definecolor{lightgray204}{RGB}{204,204,204}
\definecolor{purple}{RGB}{128,0,128}

\begin{axis}[
legend cell align={left},
legend style={
  fill opacity=0.8,
  draw opacity=1,
  text opacity=1,
  at={(0.03,0.97)},
  anchor=north west,
  draw=lightgray204
},
tick align=outside,
tick pos=left,
title={Walker-run},
x grid style={darkgray176},
xmajorgrids,
xmin=-0.95, xmax=19.95,
xtick style={color=black},
y grid style={darkgray176},
ymajorgrids,
ymin=-6.84504016124561, ymax=615.9174336598,
ytick style={color=black}
]
\path [draw=purple, fill=purple, opacity=0.2]
(axis cs:0,25.4511484999492)
--(axis cs:0,22.6288462619333)
--(axis cs:1,44.7827584248169)
--(axis cs:2,117.139122283893)
--(axis cs:3,163.08980316628)
--(axis cs:4,179.563245086508)
--(axis cs:5,201.251384750555)
--(axis cs:6,244.75725823337)
--(axis cs:7,319.790700528692)
--(axis cs:8,383.55299831238)
--(axis cs:9,416.033765830547)
--(axis cs:10,438.2478739689)
--(axis cs:11,456.034619348274)
--(axis cs:12,477.740206210838)
--(axis cs:13,493.969006647018)
--(axis cs:14,500.727071508583)
--(axis cs:15,513.722267916071)
--(axis cs:16,517.818103181349)
--(axis cs:17,519.807331864984)
--(axis cs:18,535.958459925565)
--(axis cs:19,545.574312494123)
--(axis cs:19,587.610048486116)
--(axis cs:19,587.610048486116)
--(axis cs:18,579.175152848793)
--(axis cs:17,564.67267528055)
--(axis cs:16,558.623763499644)
--(axis cs:15,553.12246718955)
--(axis cs:14,544.46022471663)
--(axis cs:13,536.741211785498)
--(axis cs:12,517.835942868398)
--(axis cs:11,493.93425339935)
--(axis cs:10,474.201771360285)
--(axis cs:9,444.330579627501)
--(axis cs:8,410.337553773948)
--(axis cs:7,373.765238406237)
--(axis cs:6,305.343881385463)
--(axis cs:5,248.786411532274)
--(axis cs:4,203.439018014689)
--(axis cs:3,167.862699480418)
--(axis cs:2,142.014340595931)
--(axis cs:1,61.0948817534479)
--(axis cs:0,25.4511484999492)
--cycle;

\path [draw=blue, fill=blue, opacity=0.2]
(axis cs:0,23.3447004423426)
--(axis cs:0,21.4623450124383)
--(axis cs:1,63.0875509133974)
--(axis cs:2,127.080427099485)
--(axis cs:3,166.064114466523)
--(axis cs:4,200.520323849594)
--(axis cs:5,253.284324354465)
--(axis cs:6,339.623916502225)
--(axis cs:7,402.197596917745)
--(axis cs:8,426.83182431667)
--(axis cs:9,446.792015498451)
--(axis cs:10,459.288954246431)
--(axis cs:11,468.76782809662)
--(axis cs:12,482.264467381517)
--(axis cs:13,496.658410184469)
--(axis cs:14,493.836078408412)
--(axis cs:15,508.572338324502)
--(axis cs:16,515.747440662534)
--(axis cs:17,511.719167294423)
--(axis cs:18,520.888034819851)
--(axis cs:19,530.098895599447)
--(axis cs:19,577.847372375081)
--(axis cs:19,577.847372375081)
--(axis cs:18,570.124639556795)
--(axis cs:17,555.847433789721)
--(axis cs:16,558.369907129332)
--(axis cs:15,548.860431270473)
--(axis cs:14,527.644084187785)
--(axis cs:13,532.136410217148)
--(axis cs:12,517.897706483223)
--(axis cs:11,505.714206977072)
--(axis cs:10,498.866408776346)
--(axis cs:9,481.663240924001)
--(axis cs:8,451.586077516399)
--(axis cs:7,417.411416430674)
--(axis cs:6,369.505396513944)
--(axis cs:5,296.261775836773)
--(axis cs:4,239.075101809043)
--(axis cs:3,171.82190150085)
--(axis cs:2,143.78826081073)
--(axis cs:1,74.3724785423547)
--(axis cs:0,23.3447004423426)
--cycle;

\path [draw=red, fill=red, opacity=0.2]
(axis cs:0,24.4591517544282)
--(axis cs:0,23.4859049848517)
--(axis cs:1,37.6499099998756)
--(axis cs:2,87.1006376024501)
--(axis cs:3,151.521494161724)
--(axis cs:4,173.858394762365)
--(axis cs:5,229.92645740259)
--(axis cs:6,283.745711473873)
--(axis cs:7,341.001937873767)
--(axis cs:8,379.151911878715)
--(axis cs:9,415.249884358656)
--(axis cs:10,437.636250398483)
--(axis cs:11,451.643007474119)
--(axis cs:12,464.977493265528)
--(axis cs:13,484.879316346113)
--(axis cs:14,487.9405248112)
--(axis cs:15,501.521776410783)
--(axis cs:16,502.272670966388)
--(axis cs:17,503.967622465835)
--(axis cs:18,516.844215703467)
--(axis cs:19,526.164134780519)
--(axis cs:19,582.190209165075)
--(axis cs:19,582.190209165075)
--(axis cs:18,575.560119217478)
--(axis cs:17,560.747572082052)
--(axis cs:16,561.662738302385)
--(axis cs:15,561.989748986029)
--(axis cs:14,540.577981757634)
--(axis cs:13,536.386811855632)
--(axis cs:12,523.596683824911)
--(axis cs:11,512.269761093302)
--(axis cs:10,501.219899297823)
--(axis cs:9,479.989735078094)
--(axis cs:8,448.540483824416)
--(axis cs:7,418.1035741664)
--(axis cs:6,348.373399047355)
--(axis cs:5,276.260261320873)
--(axis cs:4,182.732197290415)
--(axis cs:3,157.729898252668)
--(axis cs:2,115.08672740413)
--(axis cs:1,50.6777313876231)
--(axis cs:0,24.4591517544282)
--cycle;

\path [draw=green, fill=green, opacity=0.2]
(axis cs:0,26.9598805469504)
--(axis cs:0,25.6741281821679)
--(axis cs:1,43.1390681249163)
--(axis cs:2,104.540778758494)
--(axis cs:3,144.585844776062)
--(axis cs:4,172.739432376159)
--(axis cs:5,193.97890916176)
--(axis cs:6,243.441696141957)
--(axis cs:7,277.985023615247)
--(axis cs:8,301.922127139429)
--(axis cs:9,321.416691249484)
--(axis cs:10,338.083370032299)
--(axis cs:11,349.287974611783)
--(axis cs:12,345.639803433762)
--(axis cs:13,363.25185409078)
--(axis cs:14,365.280831931221)
--(axis cs:15,375.637397870454)
--(axis cs:16,376.53559490693)
--(axis cs:17,375.932709794961)
--(axis cs:18,385.083991032499)
--(axis cs:19,388.711608828541)
--(axis cs:19,439.622255309688)
--(axis cs:19,439.622255309688)
--(axis cs:18,431.317145797505)
--(axis cs:17,424.035989450968)
--(axis cs:16,425.432800977074)
--(axis cs:15,421.956271128465)
--(axis cs:14,412.754439150147)
--(axis cs:13,408.298913597291)
--(axis cs:12,390.0212486003)
--(axis cs:11,389.385673592019)
--(axis cs:10,381.637758048057)
--(axis cs:9,365.379852870027)
--(axis cs:8,348.231544887876)
--(axis cs:7,327.270974860557)
--(axis cs:6,292.840404676772)
--(axis cs:5,248.393221635911)
--(axis cs:4,216.478311423179)
--(axis cs:3,158.128052289752)
--(axis cs:2,125.900277620624)
--(axis cs:1,53.1908204997644)
--(axis cs:0,26.9598805469504)
--cycle;

\addplot [very thick, purple]
table {%
0 24.0866538722651
1 53.5924858033912
2 130.03436041794
3 165.345379817736
4 190.748258102367
5 224.413309332744
6 275.141838063084
7 347.352292462056
8 397.936844636609
9 431.068452027448
10 456.400358221965
11 475.075721075192
12 496.899352704006
13 515.569123371717
14 522.467475725185
15 533.154833634526
16 537.794324781759
17 541.64188617697
18 557.138786627935
19 567.570679684328
};
\addlegendentry{ntraj=10}
\addplot [very thick, blue]
table {%
0 22.4061201677868
1 68.9754442808037
2 135.997587657113
3 168.940963448311
4 218.721785543772
5 275.413368260661
6 355.355609771329
7 409.664753078509
8 438.954641428119
9 463.506734942879
10 478.445581078237
11 486.692147205554
12 498.172119314847
13 514.50210613348
14 510.680403389898
15 529.295105586653
16 535.825603635562
17 532.658165164301
18 543.414272327058
19 552.024718391851
};
\addlegendentry{ntraj=7}
\addplot [very thick, red]
table {%
0 23.9757107761758
1 43.9113313957473
2 100.721023372139
3 154.636890434774
4 178.275131707502
5 253.45056370647
6 316.152877712854
7 379.575722140024
8 415.904911442553
9 445.418408460614
10 469.583064174881
11 482.063994166959
12 493.764810347057
13 510.754752634255
14 514.032097857899
15 529.850050544637
16 529.857970001701
17 530.697971028688
18 544.753495594475
19 551.999652980247
};
\addlegendentry{ntraj=5}
\addplot [very thick, green]
table {%
0 26.3317017675445
1 48.3211500677476
2 114.928791243772
3 151.336154505517
4 192.676650127625
5 219.397076469541
6 266.399317076465
7 302.380776576854
8 325.781605605945
9 343.831140038165
10 361.219516109053
11 371.047231781514
12 369.240330681032
13 387.078290441054
14 389.470344008158
15 400.444830358382
16 401.670085332906
17 400.628145576747
18 410.396738127657
19 415.784751357978
};
\addlegendentry{ntraj=2}
\end{axis}

\end{tikzpicture}


==> iclr_2024/4_implementation.tex <==
\section{Implementation}

The COPILOT framework we propose is versatile and applicable to any Dyna-style MBRL algorithm. 
In this section, we are going to introduce the implementation of COPILOT on top of two popular Dyna-style MBRL algorithms: MBPO \citep{janner2019trust} for vector input and Dreamer \citep{hafner2019dream} for image input.


\subsection{COPILOT-MBPO}

\begin{equation}\label{eq_model_loss}
\resizebox{\hsize}{!}{$
\mathcal{L}(\theta) =  \sum_{n=1}^N [\mu^b_{\theta}(s_n,a_n)-s_{n+1}]^\top {\Sigma^b_{\theta}}^{-1}(s_n,a_n)[\mu^b_{\theta}(s_n,a_n)-s_{n+1}] + \log\det\Sigma^b_{\theta}(s_n,a_n)
$}
\end{equation}

\begin{algorithm}[htbp]
\caption{COPILOT-MBPO}
\begin{algorithmic}[1]
\REQUIRE interaction epochs $I$, rollout horizon $h_r$, planning horizon $h_p$, uncertainty penalty rate $\alpha_c$, uncertainty bonus rate $\alpha_o$ \
\STATE Initialize policy $\pi_\phi$, critic $V_\psi$, predictive model $\hat{\mathcal{P}}_{\theta_i}
    (i=1,..., N)$, environment model training buffer $\mathcal{D}_{\textit{e}}$, agent training buffer dataset $\mathcal{D}_{\textit{m}}$
\FOR{$I$ epochs}
    \FOR{t=1 to T}
    % \STATE Sample $k$ actions: $a^{(1)},..., a^{(2)}\sim \pi_\theta(\cdot|s_t)$
    % \FOR{}
    % \STATE Generate $k$ action candidates using policy $\pi$, planing $k$ trajectories using the learned dynamics model under planning horizon $h_p$ \
    % \STATE Compute the reward and uncertainty at each planning step \
    % \STATE Choose an action from $k$ action candidates according to Eq.\ref{eq_act_planning} to interact with the environment, add samples into real sample buffer $\mathbb{D}_e$ \ 
    \STATE Select action with uncertatinty bonus $a_t = \textbf{MPC}\big(\pi_\phi, V_\psi, s, \hat{P}_{\theta_i}
    (i=1,..., N), K, H, \alpha_b\big)$, add to $\mathcal{D}_{\textit{e}}$
    \STATE Train dynamics model $\hat{T}_\theta$ via Equation~(\ref{eq_model_loss})
    \FOR{$M$ model rollouts}
    \STATE Sample initial rollout states from real sample buffer $\mathcal{D}_{\textit{e}}$ \
        \FOR{$h=0$ to $H-1$}
            %\STATE  Select action with uncertainty penalty $\displaystyle a_{t+h} = \textbf{MPC}\big(\pi_\phi, V_\psi, s, \hat{P}_{\theta_i}(i=1,..., N), K, H, \alpha_p\big)$, rollout trained environment model and add to $\mathcal{D}_{\textit{m}}$
            \STATE $\displaystyle a_{t+h} = \textbf{MPC}\big(\pi_\phi, V_\psi, s, \hat{P}_{\theta_i}(i=1,..., N), K, H, \alpha_p\big)$ (Select action with uncerntainty penalty), rollout trained environment model and add to $\mathcal{D}_{\textit{m}}$
        \ENDFOR
    \ENDFOR
    \FOR{$G$ gradient updates}
        \STATE Update current policy $\pi$ using model-generated samples from model sample buffer $\mathcal{D}_m$ \
    \ENDFOR
    \ENDFOR
\ENDFOR
\end{algorithmic}
\end{algorithm}

\subsection{COPILOT-Dreamer}

\begin{algorithm}[htbp]
\caption{COPILOT-Dreamer}
\begin{algorithmic}[1]
\REQUIRE interaction epochs $I$, rollout horizon $h_r$, planning horizon $h_p$, uncertainty penalty rate $\alpha_p$, uncertainty bonus rate $\alpha_b$ \
\STATE Initialize policy $\pi_\phi$, critic $V_\psi$, predictive model $\hat{\mathcal{P}}_{\theta_i}
    (i=1,..., N)$, environment model training buffer $\mathcal{D}_{\textit{e}}$, agent training buffer dataset $\mathcal{D}_{\textit{m}}$
\FOR{$I$ epochs}
    \FOR{t=1 to T}
    % \STATE Sample $k$ actions: $a^{(1)},..., a^{(2)}\sim \pi_\theta(\cdot|s_t)$
    % \FOR{}
    % \STATE Generate $k$ action candidates using policy $\pi$, planing $k$ trajectories using the learned dynamics model under planning horizon $h_p$ \
    % \STATE Compute the reward and uncertainty at each planning step \
    % \STATE Choose an action from $k$ action candidates according to Eq.\ref{eq_act_planning} to interact with the environment, add samples into real sample buffer $\mathbb{D}_e$ \ 
    \STATE Select action with uncertatinty bonus $a_t = \textbf{MPC}\big(\pi_\phi, V_\psi, s, \hat{P}_{\theta_i}
    (i=1,..., N), K, H, \alpha_b\big)$, add to $\mathcal{D}_{\textit{e}}$
    \STATE Train dynamics model $\hat{T}_\theta$ via Equation~(\ref{eq_model_loss})
    \FOR{$M$ model rollouts}
    \STATE Sample initial rollout states from real sample buffer $\mathcal{D}_{\textit{e}}$ \
        \FOR{$h=0$ to $H-1$}
            %\STATE  Select action with uncertainty penalty $\displaystyle a_{t+h} = \textbf{MPC}\big(\pi_\phi, V_\psi, s, \hat{P}_{\theta_i}(i=1,..., N), K, H, \alpha_p\big)$, rollout trained environment model and add to $\mathcal{D}_{\textit{m}}$
            \STATE $\displaystyle a_{t+h} = \textbf{MPC}\big(\pi_\phi, V_\psi, s, \hat{P}_{\theta_i}(i=1,..., N), K, H, \alpha_p\big)$ (Select action with uncerntainty penalty), rollout trained environment model and add to $\mathcal{D}_{\textit{m}}$
        \ENDFOR
    \ENDFOR
    \FOR{$G$ gradient updates}
        \STATE Update current policy $\pi$ using model-generated samples from model sample buffer $\mathcal{D}_m$ \
    \ENDFOR
    \ENDFOR
\ENDFOR
\end{algorithmic}
\end{algorithm}

==> neurips_2023/1_intro.tex <==
\section{Introduction}\label{sec:intro}

\begin{wrapfigure}[10]{R}{5cm}
\vspace{-20pt}
\includegraphics[width=5cm]{MBRL-model based planning/exp/exp_total_new.png}
\vspace{-20pt}
\caption{Mean performance of \ouralgo compared with baselines across 3 diverse benchmarks.
% The performance shows a significant improvement. 
% In visual DMC tasks, COPlanner represents COPlanner-DreamerV3. In other two domains, COPlanner means COPlanner-MBPO.
}\label{fig: exp_total}
% \vspace{-15pt}
\end{wrapfigure}
Model-Based Reinforcement Learning (MBRL) has emerged as a promising approach to improve the sample efficiency of model-free RL methods. 
Most MBRL methods contain two phases that are alternated during training: 1) the first phase where the agent interacts with the real environment using a policy to obtain samples for dynamics model learning; 2) the second phase where the learned dynamics model rolls out to generate massive samples for updating the policy.
Consequently, learning an accurate dynamics model is critical as the model-generated samples with high bias can mislead the policy learning~\citep{deisenroth2011pilco, wu2022plan}.

\begin{figure}[!htbp]
\centering
\vspace{-15pt}
\includegraphics[width=0.8\textwidth]{MBRL-model based planning/exp/framework_v3.png}
\vspace{-10pt}
\caption{\small{\ouralgo Framework. The most essential part of \ouralgo is the \textit{Uncertainty-aware Policy-Guided MPC (UP-MPC) phase} in which we plan trajectories of length $H$, according to the learned dynamics model and learned policy network $\pi$, to select the action with highest trajectory reward. This UP-MPC phase is implemented differently for the two different purposes: \textit{\textcolor[RGB]{192,0,0}{environment exploration}} v.s. \textit{\textcolor[RGB]{68,114,196}{dynamics model rollouts}}. In \textcolor[RGB]{192,0,0}{environment exploration}, trajectory reward has an uncertainty bonus term to encourage exploring uncertain regions in the environment. In \textcolor[RGB]{68,114,196}{dynamics model rollouts}, trajectory reward, on the contrary, has an uncertainty penalty term to encourage policy learning on confident regions of the learned dynamics model.}}
\vspace{-20pt}
\label{fig:Framwork}
\end{figure}

However, dynamics model errors are inevitable due to the complex real-world environment.
Existing methods try to avoid model errors in two main ways.
1) Design different mechanisms such as filtering out error-prone samples to mitigate the influence of model errors after model rollouts \citep{{buckman2018sample}, {yu2020mopo}, {pan2020trust},{yao2021sample}}. 
2) Actively reduce model errors during real environment interaction through uncertainty-guided exploration \citep{{shyam2019model}, {ratzlaff2020implicit}, {sekar2020planning}, {mendonca2021discovering}}.
While both categories of methods have achieved advancements, each comes with its own set of limitations.
For the first category, although these approaches are shown to be empirically effective, they primarily concentrate on estimating uncertainty at the current step, often neglecting the long-term implications that present samples might have on model rollouts.
Moreover, post-processing samples after model rollouts can compromise rollout efficiency as many model-generated samples are discarded or down-weighted.
As for the second category, it is intrinsically challenging to achieve low model error and high long-term reward without sacrificing the sample efficiency by learning exploration policies.
% The drawback of these methods is that uncertainty-guided exploration may results in excessive investigation of areas with low rewards. 
% Samples derived from these zones will not enhance policy, resulting in low sample efficiency.

% In this paper, we propose \ouralgo, a novel model-based RL framework to improve sample efficiency in MBRL by \textit{conservative} model rollouts and \textit{optimistic} real environment exploration. More specifically, we measure the estimated model uncertainty as a penalty or a bonus on the total planning trajectory rewards for the rollout and real interaction phases respectively. We achieve this by leveraging a policy-guided model-predictive control (MPC) phase on action selection. As shown in Figure~\ref{fig:Framwork}, before each interaction with the dynamics model or the real environment, we first predict the potential future trajectories and corresponding cumulative uncertainties by performing multi-step planning with the current action. Then, Policy-Guided MPC chooses actions that either conservatively roll out imaginary trajectories to avoid model uncertain regions or optimistically explore the real environment. Conservative rollouts and optimistic exploration enjoy, interestingly, a symmetric form which makes our framework easy to implement.

To tackle the aforementioned limitations, we introduce a novel framework, \ouralgo, 
which mitigates the model errors from two aspects: 1) avoid being misled by the existing model errors via conservative model rollouts, and 2) keep reducing the model error via optimistic environment exploration. 
The two aspects are achieved simultaneously by a novel uncertainty-aware multi-step planning method, which requires no extra exploration policy training nor additional samples, resulting in stable policy updates and high sample efficiency.
% which can mitigate the influence of model errors during model rollouts and explore the environment to actively reduce model errors simultaneously by leveraging uncertainty-aware planning.
% which incorporates long-term vision and model uncertainty into action selection. 
% This innovation is unprecedented in the field of model-based RL. 
\ouralgo is structured around three core components: \textit{the Planner}, \textit{conservative model rollouts}, and \textit{optimistic environment exploration}. In the Planner, we employ an \textit{Uncertainty-aware Policy-guided Model Predictive Control} (UP-MPC) to forecast future trajectories in terms of selecting actions and to estimate the long-term uncertainty associated with each action.
% (Sec~\ref{sec: 3.1}).
As shown in Figure~\ref{fig:Framwork}, this long-term uncertainty serves as dual roles.
% tailored to mitigate the effect of model error in the two distinct phases of model-based RL: model rollouts (i.e., policy update) and environment exploration (i.e. model learning). 
% In model rollouts phase, the uncertainty guides the selection of conservative actions (Sec~\ref{sec: 3.2}), while in model learning phase, it steers towards optimistic actions for environment exploration (Sec~\ref{sec: 3.3}).
In the model rollouts phase, the uncertainty acts as a penalty on the total planning trajectory, guiding the selection of conservative actions. 
Conversely, during the model learning phase, it serves as a bonus on the total planning trajectory, steering towards optimistic actions for environment exploration.
% More specifically, we measure the estimated model uncertainty as a penalty or a bonus on the total planning trajectory rewards for the rollout and real interaction phases respectively. 
% As shown in Figure~\ref{fig:Framwork}, before each interaction with the \textcolor[RGB]{68,114,196}{dynamics model} or the \textcolor[RGB]{192,0,0}{real environment}, we first predict the potential future trajectories and corresponding cumulative uncertainties by performing multi-step planning with the current action. 
% Then, the Planner chooses actions that either \textcolor[RGB]{68,114,196}{conservatively roll out imaginary trajectories to avoid model uncertain regions} or \textcolor[RGB]{192,0,0}{optimistically explore the real environment to expand the learned model}.




Compared to previous methods, \ouralgo has the following advantages:
\textbf{(a)} \ouralgo has \textbf{higher exploration efficiency}, as it focuses on investigating high-reward uncertain regions to broaden the dynamics model, thereby preventing unnecessary excessive exploration of areas with low rewards.
\textbf{(b)} \ouralgo has \textbf{higher model-generated sample utilization rate.} Through planning for multi-step model uncertainty estimation, \ouralgo can prevent model rolled out trajectories from falling into uncertain areas, thereby avoiding model errors before model rollouts and improving the utility of model generated samples.
\textbf{(c)} \ouralgo enjoys an \textbf{unified policy framework}. Unlike previous methods \citep{{sekar2020planning}, {mendonca2021discovering}} that require training two separate policies for different usage, \ouralgo only requires training a single policy and we only change the way model-based planning is utilized, thus improving training efficiency and resolving potential policy distribution mismatches. 
\textbf{(d)} \ouralgo ensures \textbf{undistracted policy optimization}. Notably, \ouralgo diverges from existing approaches by not using long-term uncertainty as an intrinsic reward. Instead, the policy's objective remains focused on maximizing environmental rewards, thereby avoiding the introduction of spurious behaviors due to model uncertainty.


\textbf{Summary of Contributions:}
\textbf{(1)} We introduce \ouralgo framework which can mitigate the influence of model errors during model rollouts and explore the environment to actively reduce model errors simultaneously by leveraging our proposed uncertainty-aware policy-guided MPC.
\textbf{(2)} \ouralgo is a plug-and-play framework that can be applicable to any dyna-style MBRL method. 
\textbf{(3)} After being integrated with other MBRL baseline methods, \ouralgo improves the sample efficiency of these baselines by nearly double.
\textbf{(4)} Besides, \ouralgo also significantly improves the performance on a suite of proprioceptive and visual control tasks compared with other MBRL baseline methods (16.9\% on proprioceptive DMC, {32.8\% on GYM, and 9.6\% on visual DMC}).
% We propose \ouralgo framework that has a long-term vision for uncertainty estimation.
% This mechanism utilizes the long-term uncertainty for both conservative model rollouts and optimistic environment exploration, thereby addressing the inaccurate learned dynamics model problem in MBRL. 
% \textbf{(2)} More importantly, \ouralgo achieves simultaneously conservative model rollouts and optimistic environment exploration using a single policy, whose learning is not interfered by conservative rollouts or optimistic exploration, in contrast with existing works. 
% \textbf{(3)} \ouralgo is a plug-and-play framework that can be applicable to any dyna-style MBRL method. 
% \textbf{(4)} \ouralgo, combined with the current MBRL methods, significantly improves both the sample efficiency and performance on a suite of proprioceptive and visual control tasks.

==> neurips_2023/2_background.tex <==
\section{Preliminaries}
\textbf{Model-based reinforcement learning.}
We consider a Markov Decision Process (MDP) defined by the tuple $(\mathcal{S}, \mathcal{A}, \mathcal{T},\rho_0, r, \gamma)$, 
where $\mathcal{S}$ and $\mathcal{A}$ are the state space and action space respectively, $\mathcal{T}(s^{\prime}|s,a)$ is the transition dynamics, $\rho_0$ is the initial state distribution, $r(s,a)$ is the reward function and $\gamma$ is the discount factor.
In model-based RL, the transition dynamics $T$ in the real world is unknown, and we aim to construct a model $\hat{T}(s^{\prime}|s,a)$ of transition dynamics and use it to find an optimal policy $\pi$ which can maximize the expected sum of discounted rewards,
\begin{equation}
\label{eq_MBRLgoal}
\pi = \mathop{\arg\!\max}_{\pi}\mathbb{E}_{{s_{t}\sim \hat{T}(\cdot|s_{t-1},a_{t-1})} \atop{a_t \sim \pi(a|s_t)}}\left[\sum_{t=0}^{\infty}\gamma^t r(s_t, a_t)\right].
\end{equation}

\textbf{Model predictive control.}
Model predictive control (MPC) has a long history in robotics and control systems \citep{{garcia1989model}, {qin2003survey}}.
MPC find the optimal action through trajectory optimization. 
Specifically, given the transition dynamics $T$ in the real world, the agent obtains a local solution at each step $t$ by estimating optimal actions over a finite horizon $H$ (i.e., from $t$ to $t+H$) and executing the first action $a_t$ from the computed optimal sequence at time step $t$:
\begin{equation}
\label{eq_MPCgoal}
a_t = \mathop{\arg\!\max}_{a_{t:t+H}}\mathbb{E}\left[\sum_{i=t}^H \gamma^i r(s_i, a_i)\right], s_i \sim T(\cdot|s_{i-1}, a_{i-1}),
\end{equation}
where $\gamma$ is typically set to 1.
In model-based control methods, the transition dynamics $T$ is %always
simulated by the learned dynamics model $\hat{T}$ \citep{{chua2018deep}, {wang2019exploring}, {hansen2022temporal}}.

==> neurips_2023/3_method.tex <==
\section{The \ouralgo Framework}
% In this section, we will introduce our \ouralgo framework. 
% We first present the core part of \ouralgo called Policy-Guided model predictive control, or Policy-Guided MPC.
% Then we introduce the specific forms of Policy-Guided MPC for different purposes at different stages, namely model rolling out conservatively and exploring the environment optimistically.
% As motivated in previous sections that being able to avoid or reduce model error dueing planning and model learning is the major issue we aim to tackle. 
% Our idea is to adjust actions according to model uncertainty based on the curre t learned transition dynamics and current policy. the major novelty includes (1) how to calculate model uncertainty, (2) how to adjust the action selection during the two differencet stages of the model-based RL, and (3) how to select action that has a long-term vision. In this section, we will introduce a planner, which concerns the 3rd novelty. how to use this planner, which concerns the second novelty, will be introduced in the following subsections.

In this section, we will introduce \ouralgo framework. 
\ouralgo consists of three components: the Planner, conservative model rollouts, and optimistic environment exploration. 
Within the Planner, we propose using an Uncertainty-aware Policy-guided MPC to predict potential future trajectories when selecting different actions under the current state and estimate the long-term uncertainty associated with each action, which will be introduced in Sec~\ref{sec: 3.1}.
Depending on the phase, this long-term uncertainty is used to further guide the selection of conservative actions for policy learning or optimistic actions for environment exploration which will be introduced in Sec~\ref{sec: 3.2} and Sec~\ref{sec: 3.3}. 
% It's worth noting that, unlike previous works, in our framework, the long-term uncertainty is not used as an intrinsic reward for policy training.
% The policy's objective remains to maximize the environment reward, which mitigates any potential issues with the policy learning spurious behaviors due to model uncertainty.
% The pseudocode of \ouralgo is shown in Algorithm~\ref{coplanner wrapper}, and a more detailed figure is shown in Appendix~\ref{app: framework_figure}.




\subsection{``The Planner'': Uncertainty-Aware Policy-Guided MPC}\label{sec: 3.1}

\begin{wrapfigure}{r}{0.45\textwidth}
\vspace{-13pt}
\includegraphics[width=0.45\textwidth]{MBRL-model based planning/exp/MPC_v2.png}
\vspace{-10pt}
\caption{The Planner.\label{fig:mpc}}
\vspace{-18pt}
\end{wrapfigure}
In this section, we present the core part of our proposed framework which is called Uncertainty-aware Policy-guided MPC (UP-MPC). 
% \fhc{As motivated in previous sections that being able to avoid or reduce model error dueing planning and model learning is the major issue we aim to tackle. Our idea is to adjust actions according to model uncertainty based on the curret learned transition dynamics and current policy. the major novelty includes (1) how to calculate model uncertainty, (2) how to adjust the action selection during the two differencet stages of the model-based RL, and (3) how to select action that has a long-term vision. In this section, we will introduce a planner, which concerns the 3rd novelty. how to use this planner, which concerns the second novelty, will be introduced in the following subsections. }
Inspired by MPC, we apply the random shooting method \citep{rao2009survey} to introduce a long-term vision. % in MPC.
Specifically, given the current state $s_t$, before each interaction with the model or real environment, we first generate an action candidate set containing $K$ actions using the policy: $\bm{a_t} = \{a_t^{(1)}, a_t^{(2)}, ..., a_t^{(k)}\}$.
Then, for each action candidate, we perform $H_p$-step planning and calculate the reward $r$, and model uncertainty $u$ for each step.
Finally, we select the action according to accumulated reward and model uncertainty, (to interact with the learned dynamics for the model rollouts or to interact with the environment for the model learning),  
% This selected action will be used for different purposes: to interact with the model for the model rollouts phase or to interact with the environment for the environment exploration. 
as will be discussed in details in Sec~\ref{sec: 3.2} and Sec~\ref{sec: 3.3}.

Incorporating model uncertainty is crucial for action selection to compensate for model error.
As illustrated in Algorithm~\ref{alg: MPC}, we calculate the model uncertainty $u$ through the model disagreement \citep{pathak2019self} method. 
Model disagreement is closely related to model learning and is currently the most common way to estimate model uncertainty in MBRL \citep{{yu2020mopo}, {kidambi2020morel}, {pan2020trust}, {sekar2020planning}, {yao2021sample}, {mendonca2021discovering}}. 
We train a dynamics model ensemble $\hat{T}_{\theta} = \{ \hat{T}^{(1)}_{\theta}, \hat{T}^{(2)}_{\theta}, ..., \hat{T}^{(n)}_{\theta} \}$ to predict the next state given the current state-action pair $(s_t, a_t)$ as input.
Utilizing the ensemble, we approximate the model uncertainty by calculating the variance over predicted states of the different ensemble members.
This estimation closely represents the expected information gain \citep{pathak2019self}:
\vspace{-3pt}
\begin{equation}
\label{eq_model_disagreement}
u(s_t, a_t) = \frac{1}{N-1}\sum_n (\hat{T}^{(n)}_{\theta}(s_t, a_t) - \mu^{\prime})^2, \quad \mu^{\prime} = \frac{1}{N}\sum_n \hat{T}^{(n)}_{\theta}(s_t, a_t).
\end{equation}
\vspace{-10pt}

See Figure~\ref{fig:mpc} for the illustration of the process.
The pseudocode for the Planner, i.e., the UP-MPC process, is summarized in Algorithm~\ref{alg: MPC}.

\vspace{-10pt}
\begin{algorithm}[!htbp]
\caption{The Planner: \textbf{UP-MPC}\;\big($\pi_\phi$, $s$, $\hat{T}_{{\theta}}$, $K$, $H$, $\alpha$\big)}
\begin{algorithmic}[1]
\REQUIRE Policy $\pi_\phi$, State $s$, learned dynamics model $\hat{T}_{{\theta}}$, number of candidates actions $K$, planning horizon $H_p$, optimistic/conservative parameter $\alpha$ \
\STATE Initialize $R^{(k)}=0$ for $k=1,..., K$, $s^{(k)}_0=s$ for $k=1,..., K$
\FOR {$k=1$ to $K$}
\FOR{$t=0$ to $H_p-1$}
    \STATE Sample $a^{(k)}_t\sim \pi_\phi(\cdot|s^{(k)}_t)$
    \STATE Rollout dynamics model $r^{(k)}_{t} = \hat{R}(\cdot|s^{(k)}_t, a^{(k)}_t), \; s^{(k)}_{t+1}\sim \hat{T}_{{\theta}}(\cdot|s^{(k)}_t, a^{(k)}_t)$
    \STATE Compute model uncertainty $u^{(k)}_t$ according to Eq.~\ref{eq_model_disagreement}
    \STATE $R^{(k)} = R^{(k)} + r^{(k)}_t + \alpha u^{(k)}_t$
    \ENDFOR
\ENDFOR
\STATE  Select $k^*=\argmax_{k=1,..., K}R^{(k)}$
\RETURN $a^{({k^*})}_0$
\end{algorithmic}
\label{alg: MPC}
\end{algorithm}
\vspace{-5pt}

Although in  Algorithm~\ref{alg: MPC} 
% for simplicity of illustration, 
model uncertainty $u$ is implemented through model disagreement, our proposed 
UP-MPC is a generic framework, any method for calculating intrinsic rewards to encourage exploration can be embedded into our framework for computing $u$. 
In Appendix~\ref{app: exp_uncert} we provide an ablation study of uncertainty estimation methods to further illustrate this point.
% Here we only introduce the model disagreement \citep{pathak2019self} method we used. 


\subsection{Conservative model rollouts}\label{sec: 3.2}

In model-based RL, due to the limited samples available for model learning, model prediction errors are inevitable. 
If a policy is trained using model-generated samples with a large error, these samples will not provide correct gradient and may mislead the policy update. 
Previous methods estimate the model uncertainty of each sample after generation and re-weight or discarded samples with high uncertainty. 
However, re-weighting samples based on uncertainty still leads to samples with high uncertainty participating in the policy learning process, while filtering requires manually setting an uncertainty threshold, and determining the optimal threshold is difficult. 
Discarding too many samples can result in inefficient rollouts.

% Since processing samples after generation is inefficient, can we predict the impact of an action on future rollouts before executing it, thereby avoiding generating high uncertainty samples? The answer is yes. 
We apply our Planner to plan for maximizing the future reward while minimizing the model uncertainty during model rollouts before executing the action. 
After calculating the reward and model uncertainty for the $H_p$-step trajectories of $K$ action candidates (line 5 and 6 in Algorithm~\ref{alg: MPC}),  
we replace $\alpha=\textcolor{blue}{-\alpha_c}$, for a positive $\alpha_c>0$ at line 7 in Algorithm~\ref{alg: MPC}.
Mathematically, %this choice of $\alpha=-\alpha_c$ means that 
we select the action according to Eq.~\ref{eq_act_rollout} to interact with the model for model rollouts:
\begin{equation}\label{eq_act_rollout}
\resizebox{\hsize}{!}{$
a = \mathop{\arg\!\max}_{a_t \in \bm{a_t}} \left[ r(s_t, a_t) + \sum_{i=1}^{H_p} r(\hat{s}_{t+i}, \pi(\hat{s}_{t+i})) \textcolor{blue}{- \alpha_c} \sum_{i=1}^{H_p} u(\hat{s}_{t+i}, \pi(\hat{s}_{t+i})) \right], \hat{s}_{t+i} \sim \hat{T}(\cdot|\hat{s}_{t+i-1}, a_{t+i-1}).
$}
\end{equation}
The negative $-\alpha_c$ is a coefficient that adds the model uncertainty as a penalty term to the trajectory total reward. 
By employing this approach, we can prevent model rollout trajectories from falling into model-uncertain regions while obtaining samples with higher rewards.


\subsection{Optimistic environment exploration}\label{sec: 3.3}

In addition to model rollouts, another crucial part of MBRL is interacting with the real environment to obtain samples to improve the dynamics model. 
Since the main purpose of MBRL is to improve sample efficiency, we should acquire more meaningful samples for improving the dynamics model within a limited number of interactions. 
Therefore, unlike previous methods that merely aimed to thoroughly explore the environment to obtain a comprehensive model \citep{{shyam2019model}, {ratzlaff2020implicit}, {sekar2020planning}}, we do not expect the dynamics model to learn all samples in the state space. This is because many low-reward samples do not contribute to policy improvement. 
Instead, we hope to obtain samples with both high rewards and high model uncertainty to sufficiently expand the model and reduce model uncertainty.

Similar to model rollouts, we also employ our Planner in the process of selecting actions when interacting with the environment. 
However, the difference lies in that we  replace $\alpha=\textcolor{red}{\alpha_o}$, for a positive $\alpha_o>0$ at line 7 in Algorithm~\ref{alg: MPC}.
Mathematically, we choose the action with both high cumulative rewards and model uncertainty according to Eq.~\ref{eq_act_planning}, which is a symmetric form of Eq.~\ref{eq_act_rollout}. $\alpha_o$ is a hyperparameter to balance the reward and exploration.
Such an action can guide the trajectory towards regions with high rewards and model uncertainty in the real environment, thereby effectively expanding the learned dynamics model. 
\begin{equation}
\label{eq_act_planning}
\resizebox{\hsize}{!}{$
a = \mathop{\arg\!\max}_{a_t \in \bm{a_t}} \left[ r(s_t, a_t) + \sum_{i=1}^{H_p} r(\hat{s}_{t+i}, \pi(\hat{s}_{t+i})) \textcolor{red}{+ \alpha_o} \sum_{i=1}^{H_p} u(\hat{s}_{t+i}, \pi(\hat{s}_{t+i})) \right], \hat{s}_{t+i} \sim \hat{T}(\cdot|\hat{s}_{t+i-1}, a_{t+i-1})
$}
\end{equation}

In summary, by simultaneously using conservative model rollouts and optimistic environment exploration, \ouralgo effectively alleviates the model error problem in MBRL. 
As we will show in \cref{sec: exp}, this is of great help in improving the sample efficiency and performance.
The pseudocode of \ouralgo is shown in Algorithm~\ref{coplanner wrapper}, and a more detailed figure is shown in Appendix~\ref{app: framework_figure}.
Very importantly, \ouralgo achieves both conservative model rollouts and optimistic environment exploration using a single policy. Different from prior exploration methods, the policy that \ouralgo learns does not have to be an ``exploration'' policy which is inevitably suboptimal.


\begin{algorithm}[htbp]
\caption{Main Algorithm: \ouralgo}
\begin{algorithmic}[1]
\REQUIRE Interaction epochs $I$, rollout horizon $H_r$, planning horizon $H_p$, number of candidates actions $K$, conservative rate $\alpha_c$, optimistic rate $\alpha_o$ \
\STATE Initialize policy $\pi_\phi$, dynamics model $\hat{T}$, real sample buffer $\mathcal{D}_{\textit{e}}$, model sample buffer $\mathcal{D}_{\textit{m}}$
\FOR{$I$ epochs}
    % \FOR{$t=1$ to $T$}
    \WHILE{not Done}
    \STATE Select action $a_t = \textbf{UP-MPC}\big(\pi_\phi, s_t, \hat{T}_{{\theta}}, K, H_p, \textcolor{red}{\alpha_o}\big)$
    \STATE Execute in real environment, add $(s_t, a_t, r_t, s_{t+1})$ to $\mathcal{D}_{\textit{e}}$ \
    \STATE Train dynamics model $\hat{T}_{{\theta}}$ with $\mathcal{D}_{\textit{e}}$ \
    \FOR{$M$ model rollouts}
    \STATE Sample initial states from real sample buffer $\mathcal{D}_{\textit{e}}$ \
        \FOR{$h=0$ to $H_r$}
            \STATE Select action $\displaystyle \hat{a}_{t+h} = \textbf{UP-MPC}\big(\pi_\phi, \hat{s}_h, \hat{T}_{{\theta}}, K, H_p, {\textcolor{blue}{-\alpha_c}}\big)$
            \STATE Rollout learned dynamics model and add to $\mathcal{D}_{\textit{m}}$
        \ENDFOR
    \ENDFOR
    \STATE Update current policy $\pi_{{\phi}}$ with $\mathcal{D}_m$ \
    \ENDWHILE
\ENDFOR
% \ENDFOR
\end{algorithmic}
\label{coplanner wrapper}
\end{algorithm}
\vspace{-5pt}

==> neurips_2023/4_implementation.tex <==
\section{Implementation}

The COPILOT framework we propose is versatile and applicable to any Dyna-style MBRL algorithm. 
In this section, we are going to introduce the implementation of COPILOT on top of two popular Dyna-style MBRL algorithms: MBPO \cite{janner2019trust} for vector input and Dreamer \cite{hafner2019dream} for image input.


\subsection{COPILOT-MBPO}

\begin{equation}\label{eq_model_loss}
\resizebox{\hsize}{!}{$
\mathcal{L}(\theta) =  \sum_{n=1}^N [\mu^b_{\theta}(s_n,a_n)-s_{n+1}]^\top {\Sigma^b_{\theta}}^{-1}(s_n,a_n)[\mu^b_{\theta}(s_n,a_n)-s_{n+1}] + \log\det\Sigma^b_{\theta}(s_n,a_n)
$}
\end{equation}

\begin{algorithm}[htbp]
\caption{COPILOT-MBPO}
\begin{algorithmic}[1]
\REQUIRE interaction epochs $I$, rollout horizon $h_r$, planning horizon $h_p$, uncertainty penalty rate $\alpha_c$, uncertainty bonus rate $\alpha_o$ \
\STATE Initialize policy $\pi_\phi$, critic $V_\psi$, predictive model $\hat{\mathcal{P}}_{\theta_i}
    (i=1,..., N)$, environment model training buffer $\mathcal{D}_{\textit{e}}$, agent training buffer dataset $\mathcal{D}_{\textit{m}}$
\FOR{$I$ epochs}
    \FOR{t=1 to T}
    % \STATE Sample $k$ actions: $a^{(1)},..., a^{(2)}\sim \pi_\theta(\cdot|s_t)$
    % \FOR{}
    % \STATE Generate $k$ action candidates using policy $\pi$, planing $k$ trajectories using the learned dynamics model under planning horizon $h_p$ \
    % \STATE Compute the reward and uncertainty at each planning step \
    % \STATE Choose an action from $k$ action candidates according to Eq.\ref{eq_act_planning} to interact with the environment, add samples into real sample buffer $\mathbb{D}_e$ \ 
    \STATE Select action with uncertatinty bonus $a_t = \textbf{MPC}\big(\pi_\phi, V_\psi, s, \hat{P}_{\theta_i}
    (i=1,..., N), K, H, \alpha_b\big)$, add to $\mathcal{D}_{\textit{e}}$
    \STATE Train dynamics model $\hat{T}_\theta$ via Equation~(\ref{eq_model_loss})
    \FOR{$M$ model rollouts}
    \STATE Sample initial rollout states from real sample buffer $\mathcal{D}_{\textit{e}}$ \
        \FOR{$h=0$ to $H-1$}
            %\STATE  Select action with uncertainty penalty $\displaystyle a_{t+h} = \textbf{MPC}\big(\pi_\phi, V_\psi, s, \hat{P}_{\theta_i}(i=1,..., N), K, H, \alpha_p\big)$, rollout trained environment model and add to $\mathcal{D}_{\textit{m}}$
            \STATE $\displaystyle a_{t+h} = \textbf{MPC}\big(\pi_\phi, V_\psi, s, \hat{P}_{\theta_i}(i=1,..., N), K, H, \alpha_p\big)$ (Select action with uncerntainty penalty), rollout trained environment model and add to $\mathcal{D}_{\textit{m}}$
        \ENDFOR
    \ENDFOR
    \FOR{$G$ gradient updates}
        \STATE Update current policy $\pi$ using model-generated samples from model sample buffer $\mathcal{D}_m$ \
    \ENDFOR
    \ENDFOR
\ENDFOR
\end{algorithmic}
\end{algorithm}

\subsection{COPILOT-Dreamer}

\begin{algorithm}[htbp]
\caption{COPILOT-Dreamer}
\begin{algorithmic}[1]
\REQUIRE interaction epochs $I$, rollout horizon $h_r$, planning horizon $h_p$, uncertainty penalty rate $\alpha_p$, uncertainty bonus rate $\alpha_b$ \
\STATE Initialize policy $\pi_\phi$, critic $V_\psi$, predictive model $\hat{\mathcal{P}}_{\theta_i}
    (i=1,..., N)$, environment model training buffer $\mathcal{D}_{\textit{e}}$, agent training buffer dataset $\mathcal{D}_{\textit{m}}$
\FOR{$I$ epochs}
    \FOR{t=1 to T}
    % \STATE Sample $k$ actions: $a^{(1)},..., a^{(2)}\sim \pi_\theta(\cdot|s_t)$
    % \FOR{}
    % \STATE Generate $k$ action candidates using policy $\pi$, planing $k$ trajectories using the learned dynamics model under planning horizon $h_p$ \
    % \STATE Compute the reward and uncertainty at each planning step \
    % \STATE Choose an action from $k$ action candidates according to Eq.\ref{eq_act_planning} to interact with the environment, add samples into real sample buffer $\mathbb{D}_e$ \ 
    \STATE Select action with uncertatinty bonus $a_t = \textbf{MPC}\big(\pi_\phi, V_\psi, s, \hat{P}_{\theta_i}
    (i=1,..., N), K, H, \alpha_b\big)$, add to $\mathcal{D}_{\textit{e}}$
    \STATE Train dynamics model $\hat{T}_\theta$ via Equation~(\ref{eq_model_loss})
    \FOR{$M$ model rollouts}
    \STATE Sample initial rollout states from real sample buffer $\mathcal{D}_{\textit{e}}$ \
        \FOR{$h=0$ to $H-1$}
            %\STATE  Select action with uncertainty penalty $\displaystyle a_{t+h} = \textbf{MPC}\big(\pi_\phi, V_\psi, s, \hat{P}_{\theta_i}(i=1,..., N), K, H, \alpha_p\big)$, rollout trained environment model and add to $\mathcal{D}_{\textit{m}}$
            \STATE $\displaystyle a_{t+h} = \textbf{MPC}\big(\pi_\phi, V_\psi, s, \hat{P}_{\theta_i}(i=1,..., N), K, H, \alpha_p\big)$ (Select action with uncerntainty penalty), rollout trained environment model and add to $\mathcal{D}_{\textit{m}}$
        \ENDFOR
    \ENDFOR
    \FOR{$G$ gradient updates}
        \STATE Update current policy $\pi$ using model-generated samples from model sample buffer $\mathcal{D}_m$ \
    \ENDFOR
    \ENDFOR
\ENDFOR
\end{algorithmic}
\end{algorithm}

==> neurips_2023/5_experiment.tex <==
\section{Experiment}
\label{sec: exp}

In this section, we conduct experiments to investigate following questions:
(a) Can \ouralgo be applied to both proprioceptive control MBRL and visual control MBRL methods, to improve their sample efficiency and asymptotic performance?
(b) How does each component of \ouralgo impact the performance?
(c) How does \ouralgo influence model learning and model rollouts?
% (c) How robust is \ouralgo under different hyperparameters?

\subsection{Experiment on proprioceptive control tasks}
\label{subsec: prop exp}
\textbf{Baselines}: 
In this section, we conduct experiments to demonstrate the effectiveness of \ouralgo on proprioceptive control MBRL methods. 
We combine \ouralgo with MBPO~\citep{janner2019trust}, the most classic method in proprioceptive control dyna-style MBRL, and we name the combined method as \textbf{COPlanner-MBPO}. 
The implementation details can be found in Appendix~\ref{app: implementation details}.
Consequently, \textbf{MBPO} naturally becomes one of our baselines. 
{The other three baselines are \textbf{P2P-MPC}~\citep{wu2022plan}, \textbf{MEEE}~\citep{yao2021sample}, and \textbf{M2AC}~\citep{pan2020trust}.
These three methods also aim to mitigate the impact of model errors in model-based RL.
We choose one of the most popular model-free RL mtheod \textbf{D4PG}~\citep{barth2018distributed} as another baseline.
More details of P2P-MPC, MEEE, and M2AC can be found in Section~\ref{sec: related work}.}
% The other two baselines are \textbf{P2P-MPC}~\citep{wu2022plan} and \textbf{MEEE}~\citep{yao2021sample}.
% These two methods also aim to mitigate the impact of model errors in model-based RL.
% More details of P2P-MPC, MEEE, and M2AC can be found in Section~\ref{sec: related work}.
We also provide comparison with more proprioceptive control MBRL methods in Appendix~\ref{app: exp_pmbrl}.

\textbf{Environment and hyperparameter settings}:
We conduct experiments on 8 proprioceptive continuous control tasks of DeepMind Control (DMC) and 4 proprioceptive control tasks of {MuJoCo-GYM (GYM)}.
MBPO trains an ensemble of 7 networks as the dynamics model while using the Soft Actor-Critic (SAC) as the policy network. 
In COPlanner-MBPO, we adopt the setting of MBPO and directly use the dynamics model ensemble to calculate model uncertainty for action selection in Policy-Guided MPC.
{For hyperparameter setting, we set optimistic rate $\alpha_o$ to be 1, conservative rate $\alpha_c$ to be 2 in all tasks, and set action candidate number $K$, planning horizon $H_p$ equal to 5 in all tasks.}
The specific setting are shown in the Appendix~\ref{app: hyper_vdmc}. 

\begin{figure}[!htbp]
\centering
% \includegraphics[width=0.9\textwidth]{MBRL-model based planning/exp/exp_pinput.png}
\includegraphics[width=0.9\textwidth]{MBRL-model based planning/exp/exp_propinput_new.png}
\vspace{-10pt}
\caption{Experiment results of COPlanner-MBPO and other {five} baselines on proprioceptive control environments. The curves in the first eight figures originate from DM Control tasks, while those in the last four are from {GYM} tasks. The results are averaged over 8 random seeds, and shaded regions correspond to the $95\%$ confidence interval among seeds.
During evaluation, for each seed of each method, we test for up to 1000 steps in the test environment and perform 10 evaluations to obtain an average value.  
The evaluation interval is every 1000 environment steps.
}
\vspace{-15pt}
\label{fig: pinput_comparison}
\end{figure}

% \begin{figure}[!htbp]
% \centering
% \includegraphics[width=\textwidth]{MBRL-model based planning/exp/exp_mujoco.png}
% \vspace{-15pt}
% \caption{Experiment results of COPlanner-MBPO and other three baselines on MuJoCo. The results are averaged over 4 random seeds, and shaded regions correspond to the $95\%$ confidence interval among seeds.}
% \vspace{-20pt}
% \label{fig: mujoco_comparison}
% \end{figure}

\textbf{\ouralgo significantly improves the sample efficiency and performance of MBPO}:
Through the results in Figure~\ref{fig: pinput_comparison} we can find that both sample efficiency and performance of MBPO have a significant improvement after combining \ouralgo.
\textbf{(a) Sample efficiency}:
In proprioceptive control DMC, the sample efficiency is improved by $40\%$ on average compared to MBPO. 
For example, in the Walker-walk task, MBPO requires 100k steps for the performance to reach 700, while COPlanner-MBPO only needs approximately 60k steps.
In more complex {GYM} tasks, the improvement brought by \ouralgo is even more significant.
Compared to MBPO, the sample efficiency of COPlanner-MBPO has almost doubled.
\textbf{(b) Performance}:
From the performance perspective, as shown in Figure~\ref{fig: exp_total}, the performance of MBPO has improved by $16.9\%$ after combining \ouralgo. 
Moreover, it is worth noting that our method successfully solves the Walker-run task, which MBPO fails to address, further demonstrating the effectiveness of our proposed framework.
{In GYM tasks, the average performance at convergence has increased by $32.8\%$.}
% In MuJoCo tasks, the average performance at 150k environment steps has increased by $59.7\%$.
Besides, COPlanner-MBPO also outperforms other baselines.

\subsection{Experiment on visual control tasks}

\textbf{Baselines}: 
We conduct experiments to demonstrate the effectiveness of our proposed framework on visual control environments.
We integrate our algorithm with \textbf{DreamerV3}~\citep{hafner2023mastering}, the state-of-the-art Dyna-style model-based RL approach recently introduced for visual control.
% We combine \ouralgo with DreamerV3 \citep{hafner2023mastering}, the SOTA dyna-style model-based RL for visual control proposed recently.
The implementation details can be found in Appendix~\ref{app: implementation details}.
{We choose LEXA  \citep{mendonca2021discovering} as our another baseline.
LEXA uses Plan2Explore \citep{sekar2020planning} as intrinsic reward to explore the environment and learn a world model, then using this model to train a policy to solve diverse tasks such as goal achieving.
% Here we adopt LEXA on DreamerV3 to address continuous control tasks and name it as LEXA-DreamerV3.
Since pure exploration base on Plan2Explore is sample inefficient for model learning when solving specific tasks, we use the real reward provided by environment as extrinsic reward and add it to intrinsic reward provided by Plan2Explore to train the explorer.
We adopt this method on DreamerV3 and call it \textbf{LEXA-reward-DreamerV3}.
Besides, we compare our method with the SOTA model-free visual RL method \textbf{DrQV2}~\citep{yarats2021mastering}.
}
% We choose LEXA  \citep{mendonca2021discovering} as our another baseline.
% LEXA uses Plan2Explore \citep{sekar2020planning} as intrinsic reward to explore the environment and learn a world model, then using this model to train a policy to solve diverse tasks such as goal achieving.
% Here we adopt LEXA on DreamerV3 to address continuous control tasks and name it as LEXA-DreamerV3.
% Since pure exploration base on Plan2Explore is sample inefficient for model learning when solving specific tasks, we use the real reward provided by environment as extrinsic reward and add it to intrinsic reward provided by Plan2Explore to train the explorer.
% We call this baseline LEXA-reward-DreamerV3.
We also provide comparison with more visual control MBRL methods including TDMPC~\citep{hansen2022temporal} and PlaNet~\citep{hafner2019learning} in Appendix~\ref{app: exp_vmbrl}.

\begin{figure}[!htbp]
\centering
% \includegraphics[width=0.9\textwidth]{MBRL-model based planning/exp/exp_dreamerv3.png}
\includegraphics[width=0.9\textwidth]{MBRL-model based planning/exp/exp_dreamerv3_new.png}
\vspace{-10pt}
\caption{Experiment results of COPlanner-Dreamerv3 and other three baselines on pixel-input DMC. The results are averaged over 8 random seeds, and shaded regions correspond to the $95\%$ confidence interval among seeds.
During evaluation, for each seed of each method, we test for up to 1000 steps in the test environment and perform 10 evaluations to obtain an average value. 
The evaluation interval is every 1000 environment steps.
}
\vspace{-15pt}
\label{fig: visualinput_comparison}
\end{figure}



\textbf{Environment and hyperparameter settings}:
We use 8 visual control tasks of DMC as our environment.
In COPlanner-DreamerV3, we learn a latent one-step prediction dynamics model as Plan2Explore~\citep{sekar2020planning}, the ensemble size is 8.
We set action candidate number $K$ and planning horizon $H_p$ equal to 4 in all tasks.
For optimistic rate $\alpha_o$ and conservative rate $\alpha_c$, we set them to be 1 and 0.5, respectively.
All other hyperparameters remain consistent with the original DreamerV3 paper.
% due to the complexity of the visual control environment, we tune $\alpha_o$ and $\alpha_c$ for each task separately. 
% The specific setting can be found in the Appendix~\ref{app: hyper_pdmc}. 

\textbf{\ouralgo significantly improves the sample efficiency and performance of DreamerV3}:
From the experiment results in Figure~\ref{fig: visualinput_comparison}, we observe that COPlanner-DreamerV3 improves the sample efficiency and performance significantly over DreamerV3,
{and it demonstrated a significant advantage over DrQv2.
The sample efficiency of COPlanner-DreamerV3 is more than twice that of DreamerV3, and the performance is improved by 9.6\%.}
% Besides, LEXA-DreamerV3 has a low sample efficiency and do not perform well.
% This demonstrates the limitation of pure exploration when the goal is to solve specific tasks instead of learning a dynamics model applicable to a variety of tasks.
After adding real reward as extrinsic reward for explorer learning, LEXA-reward-DreamerV3 delivers performance comparable to DreamerV3 in most environments.
It outperforms DreamerV3 in Cartpole-swingup-sparse and Hopper-stand.
However, its performance and sample efficiency are still worse than COPlanner-DreamerV3, further indicates the effectiveness of \ouralgo.

\subsection{Ablation study}

In this section, we aim to investigate the impact of different components within \ouralgo on the sample efficiency and performance.
We conduct experiments on two proprioceptive control DMC tasks (Walker-stand and Walker-run) using MBPO as baseline and two visual control DMC tasks (Hopper-hop and Cartpole-swingup-sparse) with DreamerV3 as baseline.
The results are demonstrated in Figure~\ref{fig: pure study}.
Due to page limitations, we provide the ablation study on various hyperparameters of \ouralgo in Appendix~\ref{app: sec: hyper} and the ablation study of uncertainty estimation methods in Appendix~\ref{app: exp_uncert}.

\textbf{From this ablation study, we can see that effectively combining optimistic exploration and conservative rollouts is necessary to achieve the best results.}
We find that when only using optimistic exploration (COPlanner w. Explore only), the sample efficiency and performance in all tasks are significantly improved, which highlights the importance of expanding the model. 
When only using conservative rollouts (COPlanner w. Rollout only), there is some improvement in sample efficiency and performance but to a lesser extent. 
In more complex visual control tasks, only using conservative rollouts may lead to over-conservatism, resulting in an inability to learn an effective policy in sparse reward environments (as observed with a broken seed in Cartpole-swingup-sparse) or a decrease in sample efficiency during the early stages of learning (Hopper-hop).
This is reasonable because conservative rollouts may avoid high uncertainty and high reward areas to ensure the stability of policy updates. 
Moreover, without efficiently expanding the model, it is challenging to find better solutions using only conservative rollouts in complex visual control tasks.
Experimental results show that both optimistic exploration and conservative rollouts are crucial, and using either one individually can lead to an improvement in performance. 
When combining the two (as in COPlanner), we can achieve the best results, further demonstrating the effectiveness of our method.

\begin{figure}[!htbp]
\centering
\includegraphics[width=\textwidth]{MBRL-model based planning/exp/exp_co_ablation_new.png}
\vspace{-20pt}
\caption{Ablation studies of optimistic exploration and conservative rollouts on different tasks using different mbrl baselines. In the first two proprioceptive control tasks we use MBPO as baseline. For the last two visual control tasks we employ DreamerV3. The results are averaged over 8 random seeds. We can observe that the best results are achieved when combining optimistic exploration and conservative rollouts. The benefit is more pronounced in more-challenging visual tasks.}
\vspace{-10pt}
\label{fig: pure study}
\end{figure}

\subsection{Model error and rollout uncertainty analysis}

\begin{figure}[!htbp]
\centering
\includegraphics[width=0.9\textwidth]{MBRL-model based planning/exp/exp_error.png}
\vspace{-10pt}
\caption{Model learning loss and rollout uncertainty curves for \ouralgo and two other model-based RL baselines. The left four are proprioceptive control DMC tasks, and the right four are visual control
DMC tasks.}
\vspace{-15pt}
\label{fig: error study}
\end{figure}

In this section, we will investigate the impact of \ouralgo on model learning and model rollouts.
We provide the curves of how model prediction error and rollout uncertainty change as the environment step increases in Figure~\ref{fig: error study}.
We conduct experiments on two proprioceptive control DMC tasks (Cheetah-run and Walker-run) and two visual control DMC tasks (Hopper-hop and Cartpole-swingup-sparse).

\textbf{(1)} In proprioceptive control DMC, we use the MSE loss between model prediction and ground truth next state to evaluate model prediction error during training, 
while in visual control DMC, we use the KL divergence between the latent dynamics prediction and the next stochastic representation to compute latent model prediction error. 
We observe that after integrating \ouralgo in proprioceptive control tasks, the model prediction error is significantly reduced.
In more complex visual control tasks, due to obtaining more diverse samples through exploration in the early stages of training, the model prediction error of \ouralgo is higher than the baseline (DreamerV3). However, as training progresses, the model prediction error rapidly decreases, becoming significantly lower than the model prediction error of DreamerV3. 
This allows the model to fully learn from the diverse samples, leading to an improvement in policy performance.
\textbf{(2)} For the evaluation of rollouts uncertainty, we calculate the model disagreement for each sample in the model-generated replay buffer used for policy training using dynamics model ensemble. 
We find that \ouralgo significantly reduces rollout uncertainty due to conservative rollouts, suggesting that the impact of model errors on policy learning is minimized. 
This experiment further demonstrates that the success of \ouralgo is attributed to both optimistic exploration and conservative rollouts.

==> neurips_2023/6_relatedworks.tex <==
\section{Related work}\label{sec: related work}


\textbf{Mitigating model error by improving rollout strategies.} Prior methods primarily focus on using dynamics model ensembles \citep{{kurutachmodel}, {chua2018deep}} to assess model uncertainty of samples after they were generated by the model, and then 
apply weighting techniques \citep{{buckman2018sample}, {yao2021sample}}, penalties \citep{{kidambi2020morel}, {yu2020mopo}}  or filtering \citep{{pan2020trust}, {wang2022sample}} to those high uncertainty samples to mitigate the influence of model error. 
These methods only quantify uncertainty after generating the samples 
and since their uncertainty metrics are based on the current step and are myopic, these metrics can not evaluate the potential influence of the current sample on future trajectories. 
Therefore, they fail to prevent the trajectories, which is generated through model rollout on the current policy, from entering high uncertainty regions, eventually leading to a failed policy update. 
Wu et al.~\citep{wu2022plan} proposed Plan to Predict (P2P), which reverses the roles of the model and policy during model learning to learn an uncertainty-foreseeing model, aiming to avoid model uncertain regions during model rollouts. Combined with MPC, their method achieved promising results. 
However, their approach lacks effective exploration of the environment.
Branched rollout \citep{janner2019trust} and bidirectional rollout \citep{lai2020bidirectional} take advantage of small model errors in the early stages of rollouts and uses shorter rollout horizons to avoid model errors, but these approaches limit the planning capabilities of the learned dynamics model.
Besides, different model learning objectives \citep{{shen2020model}, {eysenbach2022mismatched}, {wang2022live}, {zheng2023model}} are designed to solve objective mismatch \citep{lambert2020objective} in model-based RL and further mitigate model error during model rollouts.


\textbf{Reducing model error by improving environment exploration.} Another approach to mitigate model error is to expand the dynamics model by obtaining more diverse samples through exploration during interactions with the environment. 
However, previous methods mostly focused on pure exploration, i.e., how to make the dynamics model learn more comprehensively \citep{{lowrey2018plan}, {shyam2019model}, {ratzlaff2020implicit}, {sekar2020planning}, {seyde2020learning}, {ball2020ready}, {mendonca2021discovering}, {hu2023planning}}. 
In complex environments, thoroughly exploring the entire environment is very sample-inefficient and not practical in real-world applications. 
Moreover, using pure exploration to expand the model may lead to the discovery of many low-reward samples (e.g., different ways an agent may fall in MuJoCo environment \citep{todorov2012mujoco}), which are not very useful for policy learning. 
Mendonca et al. \citep{mendonca2021discovering} proposed Latent Explorer Achiever (LEXA) which involves a explorer for exploring the environment and one achiever for solving diverse tasks based on collected samples, but the explorer and achiever may experience policy distribution shift under specific single-task settings, causing the achiever to potentially not converge to the optimal solution.


\textbf{Mitigating model error from both sides.} One most relevant work is Model-Ensemble Exploration and Exploitation (MEEE) \citep{yao2021sample} which simultaneously expands the dynamics model and reduces the impact of model error during model rollouts. During the rollout process, it uses uncertainty to weight the loss calculated for each sample to update the policy and the critic. Before interacting with the environment, they first generate $k$ action candidates and then select the action with the highest sum of Q-value and one-step model uncertainty to execute.
However, as we mentioned earlier, weighting samples cannot fundamentally prevent the impact of model errors on policy learning, and it may still mislead policy updates. Moreover, since the one-step prediction error of dynamics models is often small \citep{pan2020trust}, relying only on the sum of Q-values and one-step model uncertainty may not effectively differentiate action candidates. As a result, samples collected during interactions with the environment might not efficiently expand the model.



==> neurips_2023/7_conclusion.tex <==
\section{Conclusion and discussion}

We investigate how to effectively address the inaccurate learned dynamics model problem in MBRL. We propose \ouralgo, a general framework that can be applied to any dyna-style MBRL method. \ouralgo utilizes Uncertainty-aware Policy-Guided MPC phase to predict the cumulative uncertainty of future steps and symmetrically uses this uncertainty as a penalty or bonus to select actions for conservative model rollouts or optimistic environment exploration. In this way, \ouralgo can avoid model uncertain areas before model rollouts to minimize the impact of model error, while also exploring high-reward model-uncertain areas in the environment to expand the model and reduce model error. Experiments on a range of continuous control tasks demonstrates the effectiveness of our method. One drawback of \ouralgo is that MPC can lead to additional computational time and we provide a detailed computational time consumption in Appendix~\ref{app: exp_cost}. We can improve computational efficiency by parallelizing planning, which we leave for future work.

==> packages.tex <==
% Recommended, but optional, packages for figures and better typesetting:
\usepackage{microtype}
\usepackage{graphicx}
\usepackage{subfigure}
\usepackage{booktabs} % for professional tables
% For theorems and such
\usepackage{amsmath}
\usepackage{amssymb}
\usepackage{mathtools}
\usepackage{amsthm}

\usepackage[utf8]{inputenc} % allow utf-8 input
\usepackage[T1]{fontenc}    % use 8-bit T1 fonts

\usepackage{url}            % simple URL typesetting
\usepackage{booktabs}       % professional-quality tables
\usepackage{amsfonts}       % blackboard math symbols
\usepackage{nicefrac}       % compact symbols for 1/2, etc.
\usepackage{microtype}      % microtypography
\usepackage{xcolor}         % colors



\usepackage{algorithm}
\usepackage[noend]{algorithmic}

\usepackage{wrapfig}
\usepackage{amssymb}
\usepackage[utf8]{inputenc}
\usepackage{caption}
\usepackage{markdown}
\usepackage{multirow}
\usepackage{amsfonts}   
\usepackage{amsmath}
\usepackage{natbib}

\usepackage{url}
\usepackage{tikz}
\usepackage{pgfplots} % used for showing all the figure
\pgfplotsset{
    compat=1.5
} 

\usepgfplotslibrary{groupplots}
\usepackage{CJKutf8}
\usepackage{cancel}
\usepackage{mathtools}
\usepackage{bm}

\usepackage{soul}

% Todonotes is useful during development; simply uncomment the next line
%    and comment out the line below the next line to turn off comments
%\usepackage[disable,textsize=tiny]{todonotes}
\usepackage[textsize=tiny]{todonotes}

\usepackage{graphicx,calc}
\newlength\myheight
\newlength\mydepth
\settototalheight\myheight{Xygp}
\settodepth\mydepth{Xygp}
\setlength\fboxsep{0pt}
\newcommand*\inlinegraphics[1]{%
  \settototalheight\myheight{Xygp}%
  \settodepth\mydepth{Xygp}%
  \raisebox{-\mydepth}{\includegraphics[height=\myheight]{#1}}%
}

% hyperref makes hyperlinks in the resulting PDF.
% If your build breaks (sometimes temporarily if a hyperlink spans a page)
% please comment out the following usepackage line and replace
% \usepackage{icml2023} with \usepackage[nohyperref]{icml2023} above.

% \usepackage[colorlinks=true,linkcolor=blue,citecolor=green,urlcolor=blue]{hyperref}


% \usepackage[backref=page,colorlinks=true,linkcolor=blue,citecolor=green,urlcolor=blue]{hyperref}
% \definecolor{mydarkblue}{rgb}{0,0.08,0.45} \usepackage[backref=page,colorlinks=true,linkcolor=mydarkblue,citecolor=mydarkblue,urlcolor=mydarkblue]{hyperref}

% if you use cleveref..
\usepackage[capitalize,noabbrev]{cleveref}


% \newcommand{\theHalgorithm}{\arabic{algorithm}}
% \usepackage{subcaption}


% \DeclareMathOperator*{\argmax}{arg\,max}
% \DeclareMathOperator*{\argmin}{arg\,min}
